An intuitive multi-frequency feature representation for SO(3)-equivariant networks

The usage of 3D vision algorithms, such as shape reconstruction, remains limited because they require inputs to be at a fixed canonical rotation. Recently, a simple equivariant network, Vector Neuron (VN) has been proposed that can be easily used with the state-of-the-art 3D neural network (NN) architectures. However, its performance is limited because it is designed to use only three-dimensional features, which is insufficient to capture the details present in 3D data. In this paper, we introduce an equivariant feature representation for mapping a 3D point to a high-dimensional feature space. Our feature can discern multiple frequencies present in 3D data, which is the key to designing an expressive feature for 3D vision tasks. Our representation can be used as an input to VNs, and the results demonstrate that with our feature representation, VN captures more details, overcoming the limitation raised in its original paper.

==> experiment.tex <==
\section{Experiment}

% NOTE(ssh):
% Thing to write (following vector neurons format?)
%

% # Experiments
% List of experiments
%   ## Invariant task
%       ### Classification / Segmentation
%       - Dataset 
%           ModelNet40, ShapeNet-Part... What they consist of. Reference if preprocessed dataset is used
%       - Rotation setup
%           z/z, z/SO(3), SO(3)/SO(3)... I think it is enough to say we just followed vector neurons.
%       - Network implementation
%           Specify the number of parameters if reduced. -> Hide this????
%       - Result 1: classification        
%       - Result 2: segmentation
%       ### Occupancy network
%       - Dataset
%           ShapeNetCore and EGAD
%       - Rotation setup
%           I/I, I/SO(3), SO(3)/SO(3)...
%       - Network Implementation
%           We did not reduce the number of parameters here. -> Hide it???
%       - Result 1: ShapeNet
%           Qualitative/Quantitative
%       - Result 2: EGAD
%           Qualitative/Quantitative
%
%   ## Equivariant task
%     ### Normal estimation
%       - Dataset
%       - Experiment setup
%       - Result
%     ### Registration
%       - Dataset
%           Reused ShapeNetCore. Make sure to mention the symmetric objects.
%       - Experiment setup
%           Rotation equivariant task (not invariant)
%           Problem definition
%           Registration method (Orthogonal Procrustes problem). 
%           How we optimize in the latent space. 
%           Metric, Baselines
%       - Result 1: Uniform density
%       - Result 2: Varying density
%           ***Analysis -> Ours can distinguish perturbation and shape features? More robust??***




% In introduction
%   1. List of experiments
%   

We conduct our experiments on both SO(3)-invariant task and SO(3)-equivariant task. We use three tasks adopted from~\cite{deng2021vector}: point cloud classification (invariant), segmentation (invariant), and implicit shape reconstruction (equivariant in the encoder, invariant in the decoder) . Further, we evaluate them on three more SO(3) equivariant tasks: implicit shape regression, the normal estimation, and point cloud registration, adopted from \cite{mescheder2019occupancy}, \cite{puny2021frame}, and \cite{zhu2022correspondence}. In all subsections, we call our approach \ours{}. 


\subsection{Neural implicit reconstruction}
\label{sec:implicit_reconstruction}
%In this task, we evaluate our method on point cloud completion from the Occupancy Network\cite{mescheder2019occupancy}. 
The objective here is to reconstruct the shape, expressed with a neural implicit function, from a partial and noisy input point cloud. The architecture and training details can be found in Appendix \ref{app:architecture_details_occnet}.

\textbf{Dataset:} We assess our method using ShapeNet consisting of 13 major classes, following the categorization in \cite{deng2021vector}. The input point cloud $P$ is comprised of 300 points, sampled from each model's surface and perturbed with noise $\epsilon \sim N(0, 0.005)$. Query points for ShapeNet are uniformly sampled within the Axis-Aligned Bounding Box (AABB).

%\textbf{Setup for Train/test Data:} The setup for experimental data is inherited from Vector Neurons. Three settings for train and test data are $I/I$, $I/SO(3)$, $SO(3)/SO(3)$. $I/I$ indicates train and test with canonical poses, $I/SO(3)$ indicates train with canonical poses and test with different $SO(3)$ rotations, and $SO(3)/SO(3)$ indicates train and test with different $SO(3)$ rotations. 

%$I$ means no augmentation is applied. $SO(3)$ means arbitrary rotations in $SO(3)$ group.


% ShapeNet occupancy table
\begin{wraptable}{r}{0.5\textwidth}
\centering
% \begin{table}[htbp]
% \begin{center}
\resizebox{0.5\textwidth}{!}
{
    \begin{tabular}{c|ccc}
    Method                              & I/I           & I/SO(3)       & SO(3)/SO(3)   \\ \hline
    OccNet\cite{mescheder2019occupancy} & 71.4          & 30.9          & 58.2          \\ \hline
    VN-OccNet\cite{deng2021vector}      & 69.3          & 69.3          & 68.8          \\
    \ours{}-OccNet(Ours)                    & \textbf{71.9} & \textbf{71.9} & \textbf{71.9} \\ \hline
    \end{tabular}
}
\caption{Volumetric mIoU on ShapeNet reconstruction with neural implicits. These results are average category mean IoU over 9 classes. $I/I$ indicates train and test with canonical poses, $I/SO(3)$ indicates train with canonical poses and test with different $SO(3)$ rotations, and $SO(3)/SO(3)$ indicates train and test with different $SO(3)$ rotations.  Bold is the best performance.}
\label{table:ShapeNet_occ}
\end{wraptable}

\textbf{Results:} Table \ref{table:ShapeNet_occ} shows the volumetric mean IoU for reconstruction. As already noted in the original paper~\cite{deng2021vector}, VN-OccNet performs worse than OccNet at canonical poses. \ours{}-OccNet on the other hand, outperforms both approaches by utilizing frequency-based features. This is evident in Figure~\ref{fig:VN_EVN_recon}, where, unlike Vector Neurons, our method captures details such as the car's side mirror and chair's legs.




% \begin{table}[htbp]
% \begin{minipage}{.41\linewidth}
% \begin{center}
% \resizebox{1.0\textwidth}{!}
% {
%     \begin{tabular}{c|ccc}
%     Method                              & I/I           & I/SO(3)       & SO(3)/SO(3)   \\ \hline
%     OccNet\cite{mescheder2019occupancy} & 71.4          & 30.9          & 58.2          \\ \hline
%     VN-OccNet\cite{deng2021vector}      & 69.3          & 69.3          & 68.8          \\
%     EVN-OccNet(Ours)                    & \textbf{71.9} & \textbf{71.9} & \textbf{71.9} \\ \hline
%     \end{tabular}
% }
% \end{center}
% \caption{Volumetric mIoU on ShapeNet reconstruction with neural implicits. These results are average category mean IoU over 9 classes. Bold is the best performance.}
% \label{table:ShapeNet_occ}
% \end{minipage}
% % \hfill
% \begin{minipage}{.59\linewidth}
% \begin{center}
% \resizebox{1.0\textwidth}{!}{
% \begin{tabular}{c|cc|cc}
% dataset                           & \multicolumn{2}{c|}{ShapeNet}                        & \multicolumn{2}{c}{ModelNet40}                       \\ \hline
% train/test data                   & \multicolumn{1}{c|}{I/SO(3)}        & SO(3)/SO(3)    & \multicolumn{1}{c|}{I/SO(3)}        & SO(3)/SO(3)    \\ \hline
% PointNet \cite{qi2017pointnet}    & \multicolumn{1}{c|}{0.214}          & 0.294          & \multicolumn{1}{c|}{0.141}          & 0.112          \\
% VN-PointNet \cite{deng2021vector} & \multicolumn{1}{c|}{0.216}          & 0.219          & \multicolumn{1}{c|}{0.150}          & 0.148          \\
% FA-PointNet \cite{puny2021frame}  & \multicolumn{1}{c|}{0.208}          & 0.215          & \multicolumn{1}{c|}{0.152}          & 0.156          \\
% EVN-PointNet (Ours)               & \multicolumn{1}{c|}{0.196}          & 0.198          & \multicolumn{1}{c|}{0.125}          & 0.126          \\
% DGCNN \cite{wang2019dynamic}      & \multicolumn{1}{c|}{0.212}          & 0.170          & \multicolumn{1}{c|}{0.201}          & 0.109          \\
% VN-DGCNN \cite{deng2021vector}    & \multicolumn{1}{c|}{0.152}          & 0.152          & \multicolumn{1}{c|}{0.092}          & 0.088          \\
% FA-DGCNN \cite{puny2021frame}     & \multicolumn{1}{c|}{0.150}          & 0.153          & \multicolumn{1}{c|}{0.083}          & 0.082          \\
% EVN-DGCNN (Ours)                  & \multicolumn{1}{c|}{\textbf{0.143}} & \textbf{0.142} & \multicolumn{1}{c|}{\textbf{0.078}} & \textbf{0.079}
% \end{tabular}
% }
% \end{center}
% \caption{Test normal estimation results on the ShapeNet dataset. $1-( \bold{n}^T \hat{\bold{n}})^2$ metric is used given predicted normal $\hat{\bold{n}}$ and ground truth normal $\bold{n}$. Bold is the best performance.}
% \label{table:normal}
% \end{minipage}
% \end{table}
\begin{figure}[htb]
\centering
\includegraphics[width=0.98\textwidth]{figure/reconstruction_samples.png}
\caption{Reconstructions of meshes from point cloud inputs across three models: the original OccNet~\cite{mescheder2019occupancy} (bottom), VN-OccNet~\cite{deng2021vector} (middle), and our proposed model (top). $SO(3)$ denotes augmentation using arbitrary rotations within the $SO(3)$ group, while $I$ signifies no rotational augmentation. The notation $x/y$ implies $x$ is used for training and $y$ for testing.}
\label{fig:VN_EVN_recon}
\end{figure}


\subsection{Implicit Shape Regression}
The objective here is compression: we want to compress 3D shapes into an embedding, and then reconstruct the same shape when just given an embedding. The purpose of this experiment is to investigate how well \ours{} capture details, in particular, whether our network can learn high-frequency details and compress them to an informative latent feature.

\textbf{Dataset:} To do this, we use EGAD dataset~\cite{morrison2020egad}} comprised of 2281 shapes. EGAD dataset provides the categorization of the shapes by shape complexity level from 0 to 25, measured by the distribution of curvature across vertices. We train our model on the given dataset, and save the embeddings. We then reproduce the original shape based on just the embedding. We use OccNet as the basis model. The training point cloud $P$ is sampled following the strategy in~\ref{sec:implicit_reconstruction}. The query points are sampled both from the surface and AABB at a 9:1 ratio, with surface points perturbed by the noise $\delta \sim N(0, 0.025)$. For all models, we train with various different rotations.

\textbf{Results:} Figure \ref{fig:VN_EVN_plot_egad} the results. As we can see, as the complexity of the shape increases, the performances of VN drop significantly, while that of ours drops at a slower rate, which again demonstrates the effectiveness of our frequency-based representation. Figure \ref{fig:VN_EVN_recon_egad} shows the qualitative result at the canonical pose. Our model is able to reconstruct the high-frequency details of the training shape, while VN-OccNet and standard OccNet smooths out or miss the detail, again showing the effectiveness of the frequency-based representation.

 \begin{figure}
     \centering
     \includegraphics[width=1.0\textwidth]{figure/egad_chart.png}
     \caption{The left graph shows the volumetric IoU of OccNet, VN-OccNet, and EVN-OccNet across the complexity level in the EGAD training set. We apply rotational augmentation during both training and test time. The right graph shows EVN-OccNet's IoU improvement over VN-OccNet.}
     \label{fig:VN_EVN_plot_egad}
 \end{figure}


% \begin{table}[htbp]
\begin{wraptable}{r}{0.47\textwidth}
\centering
\vspace{-4mm}
% \begin{center}
\resizebox{0.47\textwidth}{!}{
\begin{tabular}{c|cc|cc}
dataset                           & \multicolumn{2}{c|}{ShapeNet}                        & \multicolumn{2}{c}{ModelNet40}                       \\ \hline
train/test data                   & \multicolumn{1}{c|}{I/SO(3)}        & SO(3)/SO(3)    & \multicolumn{1}{c|}{I/SO(3)}        & SO(3)/SO(3)    \\ \hline
PointNet \cite{qi2017pointnet}    & \multicolumn{1}{c|}{0.214}          & 0.294          & \multicolumn{1}{c|}{0.141}          & 0.112          \\
VN-PointNet \cite{deng2021vector} & \multicolumn{1}{c|}{0.216}          & 0.219          & \multicolumn{1}{c|}{0.150}          & 0.148          \\
FA-PointNet \cite{puny2021frame}  & \multicolumn{1}{c|}{0.208}          & 0.215          & \multicolumn{1}{c|}{0.152}          & 0.156          \\
EVN-PointNet (Ours)               & \multicolumn{1}{c|}{0.196}          & 0.198          & \multicolumn{1}{c|}{0.125}          & 0.126          \\
DGCNN \cite{wang2019dynamic}      & \multicolumn{1}{c|}{0.212}          & 0.170          & \multicolumn{1}{c|}{0.201}          & 0.109          \\
VN-DGCNN \cite{deng2021vector}    & \multicolumn{1}{c|}{0.152}          & 0.152          & \multicolumn{1}{c|}{0.092}          & 0.088          \\
FA-DGCNN \cite{puny2021frame}     & \multicolumn{1}{c|}{0.150}          & 0.153          & \multicolumn{1}{c|}{0.083}          & 0.082          \\
EVN-DGCNN (Ours)                  & \multicolumn{1}{c|}{\textbf{0.143}} & \textbf{0.142} & \multicolumn{1}{c|}{\textbf{0.078}} & \textbf{0.079}
\end{tabular}
}

% \end{center}
\caption{Test normal estimation results on the ShapeNet and ModelNet40 dataset. $1-( \bold{n}^T \hat{\bold{n}})^2$ metric is used given predicted normal $\hat{\bold{n}}$ and ground truth normal $\bold{n}$. Bold is the best performance.}\vspace{-5mm}
\label{table:normal}
% \end{table}
\end{wraptable}

\subsection{Normal Estimation}

This task requires predicting the normal direction of an input point cloud, inherently making it rotationally equivariant. 

\textbf{Dataset:} The ModelNet40~\cite{wu20153d} and ShapeNet~\cite{chang2015shapenet} datasets are used, repurposing the same train/test split from the classification and segmentation experiments. For each object, we sampled 512 random surface points.

\textbf{Setup for train/test data:} Data configurations for this task are $I/SO(3)$ and $SO(3)/SO(3)$. Here, $I$ indicates no applied augmentation, while $SO(3)$ denotes arbitrary rotations in the $SO(3)$ group.

\textbf{Metric:}
 Our evaluation metric is adopted from \cite{puny2021frame}. For assessing the predicted normal vector $\hat{\bold{n}}$ against the ground truth $\bold{n}$, we employ the metric $1-( \bold{n}^T \hat{\bold{n}})^2$. 
 % Intuitively, it measures how the predicted normals are aligned with ground truth directions.

\textbf{Results:}
 As shown in Table~\ref{table:normal}, our method outperforms both Vector Neurons and a preceding rotation-equivariant method~\cite{puny2021frame}. 


\subsection{Point cloud registration}

The aim of point cloud registration is to align two sets of $N$ points $P, \hat{P} \in \mathbb{R}^{N \times 3}$ that come from the same shape. This is formally addressed by the Orthogonal Procrustes problem~\cite{schonemann1966generalized} a rotation matrix $R \in SO(3)$ between them. However, it requires the knowledge of the correspondences between the points in $P, \hat{P}$ which is usually hard to achieve. \cite{zhu2022correspondence} proposes a different approach, which solves for the latent codes $Z, \hat{Z} \in \mathbb{R}^{C \times 3}$ of Vector Neurons instead. Following this approach, we utilize our encoder from the shape completion task (section \ref{sec:implicit_reconstruction}) to find $R$ in the feature space. The method detail can be found in Appendix \ref{app:architecture_details_reg}.

\textbf{Dataset:} In our study, we utilize the ShapeNet dataset, previously used for implicit shape reconstruction, as described in Section \ref{sec:implicit_reconstruction}. We generate two point clouds sampled from the same shape, with one being randomly rotated around the canonical origin. Unlike the studies by \cite{zhu2022correspondence} and \cite{yuan2020deepgmr}, which employ the ModelNet40 dataset and generate denser point clouds of 1,000 or 500 points, we opt for a sparser point cloud of 300 points using ShapeNet. Our experiments feature three test configurations: 1) the rotated point cloud is merely a rotated copy of the reference point cloud; 2) it is a distinct sample from the same shape; 3) it is a distinct sample from the same shape but has a density that varies between 50 and 300 points. We evaluate our methodology against three baseline approaches: VN-EquivReg \cite{zhu2022correspondence}, DeepGMR \cite{yuan2020deepgmr} following the setting of \cite{zhu2022correspondence}, and Iterative Closest Point(ICP)\cite{121791}. Due to the symmetrical characteristics of ShapeNet objects and the absence of point correspondence information, we employ Chamfer Distance (CD) as our evaluation metric and skip the training with pose error in \cite{zhu2022correspondence}.

% \begin{wraptable}{r}{0.5\textwidth}
% \vspace{-4mm}
% \centering
%     \resizebox{0.5\textwidth}{!}
%     {
%         \begin{tabular}{c|c|c|c}
%         Rotated point cloud                      & Copy             & Distinct sample  & Varying density \\ \hline
%         ICP                                      & 0.01536          & 0.01609          & 0.02059                              \\ \hline
%         DeepGMR \cite{yuan2020deepgmr}           & \textbf{0.00000} & 0.00769          & 0.01574                              \\
%         VN-EquivReg \cite{zhu2022correspondence} & \textbf{0.00000} & 0.00560          & 0.01077                              \\
%         EVN-EquivReg (Ours)                      & \textbf{0.00000} & \textbf{0.00347} & \textbf{0.00714}                     \\ \hline
%         No rotation                              & 0.00000          & 0.00310          & 0.00611                           
%         \end{tabular}
%     }
%     \captionof{table}{Registration results on the ShapeNet dataset. The metric is Chamfer Distance. Bold is the best performance.}\vspace{-2mm}
%     \label{table:point_registration}
% \end{wraptable}


\textbf{Quantitative results:} Our hypothesis posits that our architecture's heightened ability to capture input details results in consistent feature encoding and more robust point cloud registration. Table \ref{table:point_registration} validates this hypothesis. While all learning-based methods are accurate in recovering the original rotation when a rotated copy is provided, our method distinguishes itself in scenarios that involve different samples and rotations. This advantage is particularly notable when compared to VN-EquivReg\cite{zhu2022correspondence}, which serves as the Vector Neurons-based analog to our approach. In these tests, our approach consistently stays near the ground truth values. The advantage of our method becomes increasingly evident when point density is altered, offering further support for our hypothesis.

\textbf{Qualitative results:} Figure \ref{fig:point_registration_samples} presents the qualitative outcomes for point cloud registration. VN-EquivReg struggles to distinguish between similar features, like an airplane's tail and head, or the shade and base of a lamp. In contrast, our method successfully captures finer details, such as the airplane's tailplane and the lamp's cone-shaped shade.

\begin{figure}
\begin{minipage}[b]{.5\linewidth}
    \centering
    \resizebox{1.0\textwidth}{!}
    {
        \begin{tabular}{c|c|c|c}
        Rotated point cloud                      & Copy             & Distinct sample  & Varying density \\ \hline
        ICP                                      & 0.01536          & 0.01609          & 0.02059                              \\ \hline
        DeepGMR \cite{yuan2020deepgmr}           & \textbf{0.00000} & 0.00769          & 0.01574                              \\
        VN-EquivReg \cite{zhu2022correspondence} & \textbf{0.00000} & 0.00560          & 0.01077                              \\
        EVN-EquivReg (Ours)                      & \textbf{0.00000} & \textbf{0.00347} & \textbf{0.00714}                     \\ \hline
        No rotation                              & 0.00000          & 0.00310          & 0.00611                           
        \end{tabular}
    }
    \captionof{table}{Registration results on the ShapeNet dataset. The metric is Chamfer Distance. Bold is the best performance.}
    \label{table:point_registration}
\end{minipage}
\hfill
\begin{minipage}[b]{.47\linewidth}
    \centering
    \includegraphics[width=1.0\textwidth]{figure/point_registration_samples_2row.png}
    \captionof{figure}{Qualitative results of point cloud registration. Red is the point cloud in the original pose and blue is the rotated point cloud.}
    \label{fig:point_registration_samples}
\end{minipage}
\end{figure}




\subsection{Point Cloud Classification and Segmentation}

\noindent\textbf{Dataset:} For both tasks, we adopted the experimental data setup from \cite{deng2021vector}. The ModelNet40 dataset~\cite{wu20153d}, used for object classification, comprises 40 classes with 12,311 CAD models—9843 are designated for training and the remainder for testing. For the object part segmentation task, the ShapeNet dataset~\cite{chang2015shapenet} was used, containing over 30,000 models spanning 16 shape classes.

\noindent\textbf{Setup for Train/Test Data:} Data configurations are as follows: $z/z$, $z/SO(3)$, $SO(3)/SO(3)$. Here, $z$ denotes augmentation using rotations around the z-axis exclusively, while $SO(3)$ signifies arbitrary rotations within the $SO(3)$ group. The notation $x/y$ implies $x$ is used for training and $y$ for testing.

\noindent\textbf{Results:} The results of the object Table~\ref{table:classification} contains the results of the object classification experiment, showing the classification accuracy for three different augmentation strategies. Our methodology was benchmarked against multiple rotation-equivariant and -invariant methods. The methods are grouped by whether it is equivariant, invariant, or neither. In the case of rotation-equivariant methods, they originally maintain the orientation on the feature space but achieve invariance via an additional invariant layer. Even though our method is primarily rotation-equivariant, ours is only after the PaRINet\cite{chen2022devil} which is specifically designed for invariance, especially in $z/SO(3)$ and $SO(3)/SO(3)$ setups.

%Even though our method is primarily rotation-equivariant, it outperforms most of rotation-invariant models. For the segmentation task (Table~\ref{table:segmentation}), our method again shows comparable performance to invariant models, especially in $z/SO(3)$ and $SO(3)/SO(3)$ setups.


\begin{table}
\begin{minipage}{.48\linewidth}
    \begin{center}
    \resizebox{1.0\textwidth}{!}{%
        \begin{tabular}{ccccc}
                                                                & Methods                                     & $z/z$         & $z/SO(3)$     & $SO(3)/SO(3)$ \\ \hline
                                                                & \multicolumn{4}{c}{Point / mesh inputs}                       \\ \hline
        \multirow{5}{*}{Neither}                                & PointNet (\cite{qi2017pointnet})           & 85.9          & 19.6          & 74.7          \\
                                                                & PointNet++ (\cite{qi2017pointnet++})       & 91.8          & 28.4          & 85.0          \\
                                                                & PointCNN (\cite{li2018pointcnn})           & {\ul 92.5}    & 41.2          & 84.5          \\
                                                                & DGCNN (\cite{wang2019dynamic})             & 90.3          & 33.8          & 88.6          \\
                                                                & ShellNet (\cite{zhang2019shellnet})        & \textbf{93.1} & 19.9          & 87.8          \\ \hline
        \multirow{8}{*}{\shortstack[c]{Rotation-\\equivariant}} & VN-PointNet (\cite{deng2021vector})        & 77.5          & 77.5          & 77.2          \\
                                                                & VN-DGCNN (\cite{deng2021vector})           & 89.5          & 89.5          & 90.2          \\
                                                                & EVN-PointNet (Ours)                        & 88.2          & 87.8          & 88.8          \\
                                                                & EVN-DGCNN (Ours)                           & 90.5          & {\ul 90.5}    & {\ul 90.5}    \\
                                                                & SVNet-DGCNN (\cite{su2022svnet})           & 90.3          & 90.3          & 90.0          \\
                                                                & TFN (\cite{Thomas2018TensorFN})            & 88.5          & 85.3          & 87.6          \\
                                                                & Spherical-CNN (\cite{esteves2018learning}) & 88.9          & 76.7          & 86.9          \\
                                                                & $a^3$S-CNN (\cite{liu2018deep})            & 89.6          & 87.9          & 88.7          \\ \hline
        \multirow{7}{*}{\shortstack[c]{Rotation-\\invariant}}   & SFCNN (\cite{rao2019spherical})            & 91.4          & 84.8          & 90.1          \\
                                                                & RI-Conv (\cite{zhang2019rotation})         & 86.5          & 86.4          & 86.4          \\
                                                                & SPHNet (\cite{poulenard2019effective})     & 87.7          & 86.6          & 87.6          \\
                                                                & ClusterNet (\cite{chen2019clusternet})     & 87.1          & 87.1          & 87.1          \\
                                                                & GC-Conv (\cite{zhang2020global})           & 89.0          & 89.1          & 89.2          \\
                                                                & RI-Framework (\cite{li2021rotation})       & 89.4          & 89.4          & 89.3          \\
                                                                & PaRINet (\cite{chen2022devil})             & 91.4          & \textbf{91.4} & \textbf{91.4} \\ \hline
        \end{tabular}%
    }
    \end{center}
    \caption{Test classification accuracy on the ModelNet40 dataset. Bold is the best performance and underlined is the next best performance.}
    \label{table:classification}
\end{minipage}%
\hfill
\begin{minipage}{.48\linewidth}
    \begin{center}
    \resizebox{1.0\textwidth}{!}{
        \begin{tabular}{cccc}
                                                                & Methods                                    & $z/SO(3)$     & $SO(3)/SO(3)$ \\ \hline
                                                                & \multicolumn{3}{c}{Point / mesh inputs}                                    \\ \hline
        \multirow{5}{*}{Neither}                                & PointNet (\cite{qi2017pointnet})           & 38.0          & 62.3          \\
                                                                & PointNet++ (\cite{qi2017pointnet++})       & 48.3          & 76.7          \\
                                                                & PointCNN (\cite{li2018pointcnn})           & 34.7          & 71.4          \\
                                                                & DGCNN (\cite{wang2019dynamic})             & 49.3          & 78.6          \\
                                                                & ShellNet (\cite{zhang2019shellnet})        & 47.2          & 77.1          \\ \hline
        \multirow{6}{*}{\shortstack[c]{Rotation-\\equivariant}} & VN-PointNet (\cite{deng2021vector})        & 72.4          & 72.8          \\
                                                                & VN-DGCNN (\cite{deng2021vector})           & 81.4          & 81.4          \\
                                                                & EVN-PointNet (Ours)                        & 82.7          & 82.1          \\
                                                                & EVN-DGCNN (Ours)                           & {\ul 83.4}    & {\ul 83.5}    \\
                                                                & SVNet-DGCNN (\cite{su2022svnet})           & 81.4          & 81.4          \\
                                                                & TFN (\cite{Thomas2018TensorFN})            & 76.8          & 76.2          \\ \hline
        \multirow{5}{*}{\shortstack[c]{Rotation-\\invariant}}   & RI-Conv (\cite{zhang2019rotation})         & 75.3          & 75.3          \\
                                                                & GC-Conv (\cite{zhang2020global})           & 77.2          & 77.3          \\
                                                                & RI-Framework (\cite{li2021rotation})       & 79.2          & 79.4          \\
                                                                & PaRINet (\cite{chen2022devil})             & \textbf{83.8} & \textbf{83.8} \\
                                                                & TetraSphere (\cite{melnyk2022tetrasphere}) & 82.3          & 82.1          \\ \hline
        \end{tabular}
    }
    \end{center}
    \caption{Test part segmentation results on the ShapeNet dataset. These results are average category mean IoU over 16 classes. Bold is the best performance and underlined is the next best performance.}
    \label{table:segmentation}
\end{minipage}

\end{table}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
% \begin{table}[htbp]
% \begin{center}
% \resizebox{0.48\textwidth}{!}{%
% \begin{tabular}{ccccc}
%                                       & Methods                                     & $z/z$         & $z/SO(3)$     & $SO(3)/SO(3)$ \\ \hline
%                                       & \multicolumn{4}{c}{Point / mesh inputs}                       \\ \hline
% \multirow{5}{*}{Neither}              & PointNet (\cite{qi2017pointnet})           & 85.9          & 19.6          & 74.7          \\
%                                       & PointNet++ (\cite{qi2017pointnet++})       & 91.8          & 28.4          & 85.0          \\
%                                       & PointCNN (\cite{li2018pointcnn})           & {\ul 92.5}    & 41.2          & 84.5          \\
%                                       & DGCNN (\cite{wang2019dynamic})             & 90.3         & 33.8          & 88.6          \\
%                                       & ShellNet (\cite{zhang2019shellnet})        & \textbf{93.1} & 19.9          & 87.8          \\ \hline
% \multirow{8}{*}{Rotation-equivariant} & VN-PointNet (\cite{deng2021vector})        & 77.5          & 77.5          & 77.2          \\
%                                       & VN-DGCNN (\cite{deng2021vector})           & 89.5          & 89.5          & 90.2          \\
%                                       & EVN-PointNet (Ours)                        & 88.2          & 87.8          & 88.8          \\
%                                       & EVN-DGCNN (Ours)                           & 90.5          & {\ul 90.5}    & {\ul 90.5}    \\
%                                       & SVNet-DGCNN (\cite{su2022svnet})           & 90.3          & 90.3          & 90.0          \\
%                                       & TFN (\cite{Thomas2018TensorFN})            & 88.5          & 85.3          & 87.6          \\
%                                       & Spherical-CNN (\cite{esteves2018learning}) & 88.9          & 76.7          & 86.9          \\
%                                       & $a^3$S-CNN (\cite{liu2018deep})            & 89.6          & 87.9          & 88.7          \\ \hline
% \multirow{7}{*}{Rotation-invariant}   & SFCNN (\cite{rao2019spherical})            & 91.4          & 84.8          & 90.1          \\
%                                       & RI-Conv (\cite{zhang2019rotation})         & 86.5          & 86.4          & 86.4          \\
%                                       & SPHNet (\cite{poulenard2019effective})     & 87.7          & 86.6          & 87.6          \\
%                                       & ClusterNet (\cite{chen2019clusternet})     & 87.1          & 87.1          & 87.1          \\
%                                       & GC-Conv (\cite{zhang2020global})           & 89.0          & 89.1          & 89.2          \\
%                                       & RI-Framework (\cite{li2021rotation})       & 89.4          & 89.4          & 89.3          \\
%                                       & PaRINet (\cite{chen2022devil})             & 91.4          & \textbf{91.4} & \textbf{91.4} \\ \hline
% \end{tabular}%
% }
% \end{center}
% \caption{Test classification accuracy on the ModelNet40 dataset. Bold is the best performance and underlined is the next best performance.}
% \label{table:classification}
% \end{table}



% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \begin{table}[htbp]
% \begin{center}
% \resizebox{0.48\textwidth}{!}{
%     \begin{tabular}{cccc}
%                                           & Methods                                    & $z/SO(3)$     & $SO(3)/SO(3)$ \\ \hline
%                                           & \multicolumn{3}{c}{Point / mesh inputs}                                    \\ \hline
%     \multirow{5}{*}{Neither}              & PointNet (\cite{qi2017pointnet})           & 38.0          & 62.3          \\
%                                           & PointNet++ (\cite{qi2017pointnet++})       & 48.3          & 76.7          \\
%                                           & PointCNN (\cite{li2018pointcnn})           & 34.7          & 71.4          \\
%                                           & DGCNN (\cite{wang2019dynamic})             & 49.3          & 78.6          \\
%                                           & ShellNet (\cite{zhang2019shellnet})        & 47.2          & 77.1          \\ \hline
%     \multirow{6}{*}{Rotation-equivariant} & VN-PointNet (\cite{deng2021vector})        & 72.4          & 72.8          \\
%                                           & VN-DGCNN (\cite{deng2021vector})           & 81.4          & 81.4          \\
%                                           & EVN-PointNet (Ours)                        & 81.2          & 82.1          \\
%                                           & EVN-DGCNN (Ours)                           & {\ul 83.4}    & {\ul 83.5}    \\
%                                           & SVNet-DGCNN (\cite{su2022svnet})           & 81.4          & 81.4          \\
%                                           & TFN (\cite{Thomas2018TensorFN})            & 76.8          & 76.2          \\ \hline
%     \multirow{5}{*}{Rotation-invariant}   & RI-Conv (\cite{zhang2019rotation})         & 75.3          & 75.3          \\
%                                           & GC-Conv (\cite{zhang2020global})           & 77.2          & 77.3          \\
%                                           & RI-Framework (\cite{li2021rotation})       & 79.2          & 79.4          \\
%                                           & PaRINet (\cite{chen2022devil})             & \textbf{83.8} & \textbf{83.8} \\
%                                           & TetraSphere (\cite{melnyk2022tetrasphere}) & 82.3          & 82.1          \\ \hline
%     \end{tabular}
% }
% \end{center}
% \caption{Test part segmentation results on the ShapeNet dataset. These results are average category mean IoU over 16 classes. Bold is the best performance and underlined is the next best performance.}
% \label{table:segmentation}
% \end{table}


% \begin{table}[htbp]
% \begin{center}
% \resizebox{0.5\textwidth}{!}
% {
%     \begin{tabular}{c|c|c|c}
%     Rotated point cloud                      & Copy             & Distinct sample  & Varying density \\ \hline
%     ICP                                      & 0.01536          & 0.01609          & 0.02059                              \\ \hline
%     DeepGMR \cite{yuan2020deepgmr}           & \textbf{0.00000} & 0.00769          & 0.01574                              \\
%     VN-EquivReg \cite{zhu2022correspondence} & \textbf{0.00000} & 0.00560          & 0.01077                              \\
%     EVN-EquivReg (Ours)                      & \textbf{0.00000} & \textbf{0.00347} & \textbf{0.00714}                     \\ \hline
%     No rotation                              & 0.00000          & 0.00310          & 0.00611                           
%     \end{tabular}
% }
% \end{center}
% \caption{Registration results on the ShapeNet dataset. The metric is Chamfer Distance. Bold is the best performance.}
% \label{table:point_registration}
% \end{table}

% \begin{figure}[h]
% \centering
% \includegraphics[width=0.4\textwidth]{figure/point_registration_samples.png}
% \caption{Qualitative results of point cloud registration. Red is the point cloud in the original pose and blue is the different point cloud from the same shape with the rotation applied.}
% \label{fig:point_registration_samples}
% \end{figure}


==> intro.tex <==


\begin{figure}[h]
\centering
\includegraphics[width=0.98\textwidth]{figure/reconstruction_samples.png}
\caption{Reconstructions of meshes from point cloud inputs across three models: the original OccNet~\cite{mescheder2019occupancy} (bottom), VN-OccNet~\cite{deng2021vector} (middle), and our proposed model (top).}
\label{fig:VN_EVN_recon}
\end{figure}

\section{Introduction}

% % equivariant networks and limitation of the previous point processing networks
% A rotational equivariant network is a network which meets equivariant property described as $f(Rx)=R\circ f(x)$ where $f$ is a neural network, $R\in SO(3)$ is rotation, $x\in \mathbb{R}^3$ is given 3-dimensional vector, and $\circ$ is rotation operator defined in feature space.
% These networks are beneficial when we want to process point clouds because we can exploit the rotational symmetricity of the data. For example, the performance of non-equivariant point processing network counterpart dramatically decreases by augmenting random rotation to the point clouds inputs across many tasks such as part segmentation~\cite{}, shape classification~\cite{}, normal estimation~\cite{puny2021frame}, and shape reconstruction~\cite{}. On the other hand, equipping rotational equivariant can effectively eliminate the effects of rotational augmentation and make the model outperform non-equivariant counterparts in cases where canonical orientation is not assumed.



% % one example is TFN and SE(3) transformer - summary and limitations
% Previous representative instances of the equivariant networks are TFN~\cite{Thomas2018TensorFN}, SE(3)-Transformer~\cite{fuchs2020se}, and Vector Neuron~\cite{deng2021vector}. TFN and SE(3)-Transformer builds a sophisticated graph-based architecture by borrowing the concepts from quantum mechanics~\cite{} such as spherical harmonic and Wigner-D matrix. 
% They keep the equivariant feature space by controlling rotation order, which defines the dimension of the intermediate and final feature space while keeping equivariance. As demonstrated in \cite{Chatzipantazis2022SE3EquivariantAN, Thomas2018TensorFN}, we can improve the performance of the equivariant networks by increasing the dimension of feature space.

% However, there are several limitations in these works. First, they heavily relies of their architecture relies on Clebsch–Gordan (CG) tensor product~\cite{} to have learnable parameters with the equivariant property. CG tensor project involves intensive computation of the Kronecker product, which reduces the computational efficiency in the training and test stage. Additionally, the dependency of the CG tensor product blocks its network structure from adopting recent evolving techniques of the point processing networks~\cite{}. Lastly, the understanding of those networks requires a background in quantum mechanics, which prevents active extension of the research.



% % Vector Nuerons as one representative examples: benefits, and performance
% Alternatively, an equivariant network with Vector Neurons (VN)~\cite{deng2021vector} is free from the aforementioned limitations by keeping the \textit{vectors} in the neurons and developing the Linear and non-linearity layers compatible with them to build sequential VN-version Multilayered Perceptrons (MLP). On top of these novel neurons and operators, they show that the VN can be adapted to the conventional point processing network such as PointNet~\cite{} and DGCNN~\cite{}. Additionally, the network structure is relatively easy to grasp because it requires basic knowledge of linear algebra.



% % limitation of Vector Neurons - limited feature space 3-D, as a lens of rotation order in the TFN
% Although VN has several benefits over TFN, we find that VN has a performance bottleneck due to limited feature space. In the lens of TFN, VN can be seen as a specific instance of TFN with 3-dimensional feature space without CG product~\cite{}. However, as demonstrated in \cite{} utilizing high-dimensional feature space is critical for the performance.



% % we propose new architecture which can adopt benefits of vector neurons while not limiting feature space as TFN did 1. easy to integrate framework to the conventional point processing network such as PointNet and DGCNN 2. easy to understand (?)
% Based on this observation, we propose a framework that can extend the feature dimension of vector neurons to high-dimensional space. To come up with rotational equivariance in high-dimensional space, we first define the rotation operator in that space and then develop a mapping that converts 3-dimensional vectors into $n$-dimensional ones where $n$ is the target dimension. This can be summarized to developing two functions: $\bold{D}(\cdot):SO(3) \rightarrow \mathbb{R}^{n\times n}$ and $\bold{\phi}(\cdot):\mathbb{R}^3 \rightarrow \mathbb{R}^n$ which meets $\phi(Rx)=D(R)\phi(x)$. Notably, the derivation can be described with minimal involvement of knowledge from quantum mechanics, so relatively easy to understand.

% Based on the design of $\bold{D}$ and $\bold{\phi}$, we demonstrate that they can be easily adapted to the conventional point processing network with a few lines of modification of the code. We instantiate EV-PointNet and EV-DGCNN, which integrate our framework into PointNet and DGCNN respectively.
% Finally, we show that integration of our framework to the conventional point processing network can effectively introduce rotational equivariant property while improving performance compared to previous equivariant networks including VN in several tasks such as shape classification, part segmentation, normal estimation, shape reconstruction, and pose estimation. Especially for the pose estimation, the proposed model outperforms previous methods by a large margin because ours can encode details of the shapes.



% GPT written
A rotational equivariant network upholds the equivariant property expressed as $f(Rx)=R\circ f(x)$, where $f$ denotes a neural network, $R$ signifies rotation from $SO(3)$, $x$ is a 3-dimensional vector, and $\circ$ represents the rotation operator in the feature space. Such networks are indispensable for point cloud processing, tapping into the rotational symmetry inherent to the data. Notably, non-equivariant networks often falter when subject to random rotation in tasks like part segmentation~\cite{deng2021vector}, shape classification~\cite{zhu2023e2pn}, normal estimation~\cite{puny2021frame}, and shape reconstruction~\cite{chen20223d}. Conversely, networks with rotational equivariance are resilient to these rotations and often outperform their non-equivariant counterparts, especially when no canonical orientation is assumed.

Historically, noteworthy examples of equivariant networks include TFN~\cite{Thomas2018TensorFN}, SE(3)-Transformer~\cite{fuchs2020se}, and Vector Neuron~\cite{deng2021vector}. Both TFN and the SE(3)-Transformer harness quantum mechanics concepts~\cite{sakurai1995modern}, like spherical harmonics and the Wigner-D matrix, to construct intricate graph-based designs. Their unique approach to preserving the equivariant feature space involves managing the rotation order, which influences the dimensionality of the intermediate and end feature spaces. Indeed, as shown in \cite{Chatzipantazis2022SE3EquivariantAN, Thomas2018TensorFN}, performance can be enhanced by amplifying this feature space dimension.

Nevertheless, these architectures are not free from constraints. They depend heavily on the Clebsch–Gordan (CG) tensor product~\cite{} to maintain learnable parameters with the equivariant trait. This CG reliance incurs substantial computational costs, diminishes efficiency during training and testing, and can be a barrier to incorporating emerging point processing network techniques~\cite{}. Furthermore, a foundational understanding of quantum mechanics is almost obligatory for meaningful engagement, hindering broader research proliferation.

In contrast, the Vector Neurons-based equivariant network sidesteps these limitations. By retaining vectors within neurons and devising compatible linear and non-linearity layers, it fosters the creation of sequential VN-embedded Multilayered Perceptrons (MLP). This architecture not only melds seamlessly with prevalent point processing networks like PointNet~\cite{qi2017pointnet} and DGCNN~\cite{wang2019dynamic}, but it's also more intuitively understood due to its foundation in basic linear algebra.

However, Vector Neurons, despite their advantages, are stymied by a constrained feature space. When viewed through the TFN lens, Vector Neurons resemble a TFN derivative, albeit constrained to a 3-dimensional space without the encumbrance of the CG product~\cite{zhu2023e2pn}. But, as documented, the breadth of the feature space can be pivotal for performance, so the performance of VN can be limited. 
This limitation manifested in our point completion experiment. As depicted in figure \ref{fig:VN_EVN_recon}, the quality of the reconstructed shapes via VN-OccNet lags behind the OccNet~\cite{mescheder2019occupancy} baseline.

We discovered that the equivariant components used in VN-MLP are not confined to just 3-dimensional vectors but can extend to n-dimensional vectors. By first expanding the dimension of input points from 3 to n before feeding them into VN's layers and maintaining subsequent layers as in VN, we can enhance the intermediate neuron vectors' dimensionality. This approach harnesses the benefits of a high-dimensional feature space, overcoming VN's limitations without compromising its merits.

The crux of the matter lies in determining how to escalate the feature dimension from a 3-dimensional space to an n-dimensional one while retaining the equivariant property. This translates into formulating a mapping, $\phi(\cdot): \mathbb{R}^3 \rightarrow \mathbb{R}^n$, that adheres to the equivariant property $\phi(Rx)=R\circ \phi(x)$, ensuring network-wide equivariance. We must then conceptualize "rotation" in this expanded dimensionality. And for compatibility with VN's layers, rotation application must employ matrix multiplication. To actualize the feature dimension expansion in VN, we first determine the criteria for a rotation matrix in this expansive dimension and then introduce a mapping $D(\cdot): SO(3)\rightarrow \mathbb{R}^{n\times n}$ that transitions any rotation matrix to its $n \times n$ dimensional counterpart. Subsequently, we shape $\phi$ to fulfill $\phi(Rx)=D(R)\phi$. This entire formulation requires minimal grounding in quantum mechanics, making it widely accessible.

Building upon this foundation, we demonstrate the ease with which our proposed methodology integrates into standard point processing architectures, necessitating only minimal alterations to the existing code. The resulting frameworks, EV-PointNet and EV-DGCNN, stand as testament to our approach's efficacy. Our empirical evaluations underscore the dual advantage of our technique: it not only enforces rotational equivariance but also enhances overall performance across a diverse range of tasks—from shape classification, part segmentation, and normal estimation, to point completion. Notably, infusing our expanded feature methodology into VN culminates in performance metrics that rival—even under canonical orientations—the original model's capabilities. This distinction is especially noteworthy in the realm of equivariant network research, given the common observation that the performance of equivariant structures typically lags behind that of their non-equivariant peers when dealing with aligned datasets. A detailed qualitative analysis further illuminates how our expanded feature dimensions capture the nuanced intricacies of shapes in point completion assignments, as vividly illustrated in figure \ref{fig:VN_EVN_recon}.

Furthermore, we delve into the implications of augmenting feature dimensions in the context of the correspondence-free orientation estimation task, as described by Zhu et al.~\cite{zhu2022correspondence}. This task intrinsically harnesses the equivariance characteristic: when presented with reference and target point clouds of an identical object, the objective becomes pinpointing the relative rotation between the two. As Zhu et al. emphasize, the relative rotation derived within the embedding domain can be coherently mapped to the actual point clouds owing to equivariance. This task not only mandates a holistic, rather than granular, embedding of point clouds while maintaining equivariance but also seeks a superior embedding enriched with details crucial for deducing the relative pose. Our findings resonate with the superiority of our approach: we decidedly eclipse VN benchmarks, which underlines our assertion that dimension expansion facilitates a more refined shape embedding in comparison to traditional VN.

% On this foundation, we illustrate how our methodology seamlessly integrates into conventional point processing networks with trivial code modifications. The outcomes are EV-PointNet and EV-DGCNN. Our empirical assessments highlight the potency of our technique, which both instills rotational equivariance and bolsters performance across a gamut of tasks, from shape classification and part segmentation to normal estimation and point completion. Remarkably, integrating our feature expansion into VN renders performance levels that challenge the original architecture when used with canonical orientations. To the best of our knowledge, this achievement is unprecedented in equivariant network research, as typically, the performance of equivariant networks lags behind their non-equivariant counterparts when datasets are aligned. A qualitative inspection reveals that feature dimension expansion revives intricate shape details in point completion tasks, as showcased in figure \ref{fig:VN_EVN_recon}. 

% Moreover, we investigate the effects of expanding feature dimensions in correspondence-free orientation estimation task~\cite{zhu2022correspondence}. The task explicitly utilizes the equivariance property: given reference and target point clouds of the same object, the task is to obtain relative rotation between them, and \cite{zhu2022correspondence} shows that the relative rotation obtained in the embedding space can be directly transferred to the point clouds by equivariance. This task requires not only global embedding (not point-wise embedding) of the point clouds ensuring equivariance, but also better embedding having more information about the shape to infer relative pose. 
% The results shows that ours significantly outperforms VN baselines, which demonstrates that through expanding feature dimensions we could have better embedding for the shapes than one from VN.


% Fortunately, we find that VN's equivariant components to build VN-MLP are not limited to the 3-dimensional vectors but n-dimensional ones too. Then, the idea is that before feeding points to the VN's layers we first expand the dimension of points from 3 to n, and then the afterward layers remain the same with VN. This strategy leads to an increase in the dimension of the vectors consisting of intermediate neurons so that the model could benefit from high-dimensional feature space. This idea will resolve the limitation of VN while preserving its advantages.

% Now the problem is how we can increase feature dimension from 3-dimensional space to n-dimensional space while preserving equivariant property, which can be expressed as a mapping $\phi(\cdot): \mathbb{R}^3 \rightarrow \mathbb{R}^n$. The important constraint of the $\phi$ is that it must have an equivariant property $\phi(Rx)=R\circ \phi(x)$ to make the entire network preserve equivariance. Then, we should define \textit{rotation} in high-dimensional space, and to be compatible with the VN's layers, the form of applying rotation must be matrix multiplication. Therefore, to realize expanding feature dimensions of VN, we first organize the conditions to be a rotation matrix in high dimensional space, and define a mapping $D(\cdot): SO(3)\rightarrow \mathbb{R}^{n\times n}$ which maps any rotation matrix into the rotation matrix in $n \times n$ dimensions. After that, we define $\phi$ to have $\phi(Rx)=D(R)\phi$ to be used to expand feature dimensions in VN. Note that we build this derivation with minimal quantum mechanics understanding, so it is relatively accessible.


% Building upon this, we exemplify its easy adaptation to mainstream point processing networks with minimal code alterations, resulting in EV-PointNet and EV-DGCNN. Empirical evaluations underscore the efficacy of our approach, which not only introduces rotational equivariance but also enhances performance in tasks like shape classification, part segmentation, normal estimation, and point completion. 
% Surprisingly, introducing our feature expansion method to VN makes the performance competitive to the performance of original architecture with canonical orientations. As far as we know, this is the first equivariant network work to show this, because the performance of the equivariant network is usually behind the performance of the non-equivariant one with the aligned dataset. Qualitatively, we show that expanding feature dimension recover detail shapes in point completion tasks as described in figure \ref{fig:VN_EVN_recon}. Additionally, we demonstrate that this ability to encode details of the shape leads to significant improvement in pose estimation tasks, which makes the proposed one significantly outperform VN baseline.

% \begin{table}[ht]
% \centering
% \begin{tabularx}{\linewidth}{|l|X|X|}
% \hline
%  & \textbf{High-Dim. Space} & \textbf{Integration to PPN} \\
% \hline
% \textbf{TFN~\cite{Thomas2018TensorFN}} & yes & no \\
% \hline
% \textbf{VN~\cite{deng2021vector}} & no & yes \\
% \hline
% \textbf{Ours} & yes & yes \\
% \hline
% \end{tabularx}
% \caption{Comparison with previous works}
% \label{table:comparison}
% \end{table}


==> intro_v2.tex <==

\begin{figure}[h]
\centering
\includegraphics[width=0.98\textwidth]{figure/reconstruction_samples.png}
\caption{Reconstructions of meshes from point cloud inputs across three models: the original OccNet~\cite{mescheder2019occupancy} (bottom), VN-OccNet~\cite{deng2021vector} (middle), and our proposed model (top).}
\label{fig:VN_EVN_recon}
\end{figure}

\section{Introduction}

\begin{comment}
1. we have known that high-dimensional space for the equivariant network are beneficial (TFN, others)
2. the problem is that, it is really hard to access that functions without having deep understanding of quantum mechanics 
    2-1. for example, it is hard to grasp why they have equivariant property

we organized the minimal concept needed for feature augmentation with equivariance network:
    it is rotation matrix in high-dimensional space
    and feature mapping corresponding to this rotation matrix


    
3. on the other hand, VN is beneficial it is free from the knowledge of quantum mechanics and it is easily accessible only requiring basic concepts of linear algebra
4. therefore, we organized the conditiones to be beneficial feature augmentation method in equivariant networks, which concluded to be wigner-D matrix and spherical harmonics
5. by viewing spherical harmonics as a beneficial feature augmentations, we can construct high-dim space with equivariance, but it is 

\end{comment}

% our task: feature augmentation in equivariance network
% Rotational equivariant networks ensure that even when we rotate a 3D point cloud, the network's output also rotates in a consistent manner. This makes them very useful for working with 3D shapes. Especially, they shine when these 3D data points are randomly rotated, like in tasks such as segmenting parts, classifying shapes, estimating directions, or rebuilding shapes.

% A rotational equivariant network upholds the equivariant property expressed as $f(Rx)=R\circ f(x)$, where $f$ denotes a neural network, $R$ signifies rotation from $SO(3)$, $x$ is a 3-dimensional vector, and $\circ$ represents the rotation operator in the feature space. 
Rotational equivariant networks ensure that even when we rotate a 3D point cloud, the network's output also rotates in a consistent manner.
Such networks are indispensable for point cloud processing, tapping into the rotational symmetry inherent to the data. Notably, non-equivariant networks often falter when subject to random rotation in tasks like part segmentation~\cite{deng2021vector}, shape classification~\cite{zhu2023e2pn}, normal estimation~\cite{puny2021frame}, and shape reconstruction~\cite{chen20223d}. Conversely, networks with rotational equivariance are resilient to these rotations and often outperform their non-equivariant counterparts, especially when no canonical orientation is assumed.

% On the other hand, feature augmentation is critical to the performance of the task and it is known to improve the capability to capture high-frequency features in the images and 3D shapes~\cite{mildenhall2021nerf, tancik2020fourier}. Even with the importance of both equivariant networks and feature augmentation methods, the accessible study to combine those two things is hard to find. Therefore, in this work, we seek a beneficial feature augmentation method for the equivariant point processing networks.

Simultaneously, feature augmentation plays a pivotal role in enhancing task performance, particularly in amplifying the ability to discern high-frequency features in images and 3D shapes~\cite{mildenhall2021nerf, tancik2020fourier}. Despite the recognized importance of both equivariant networks and feature augmentation, comprehensive studies integrating the two remain sparse. Motivated by this gap, our research endeavors to devise an effective feature augmentation strategy tailored for equivariant point processing networks.

% challenges in feature augmentation
The crux of the matter lies in determining how to escalate the feature dimension from a 3-dimensional space to an n-dimensional one while retaining the equivariant property. This translates into formulating a mapping, $\phi(\cdot): \mathbb{R}^3 \rightarrow \mathbb{R}^n$, that adheres to the equivariant property $\phi(Rx)=R\circ \phi(x)$, ensuring network-wide equivariance. We must then conceptualize "rotation" in this expanded dimensionality.

% previous work and limitations
Earlier, TFN~\cite{Thomas2018TensorFN} employed the Wigner-D matrix and spherical harmonics for feature augmentation in equivariant networks. In their approach, rotation in higher-dimensional space was characterized using the Wigner-D matrix, with the associated mapping defined via spherical harmonics. However, comprehending this approach necessitates a profound understanding of quantum mechanics, which limits its accessibility.

% address this, and propose new methods
To address the challenges faced with feature augmentation in equivariant networks,  we aim to devise a more accessible method, reducing the reliance on advanced quantum mechanics knowledge. While establishing the foundational conditions for feature augmentation that's suited for high-dimensional space is a start, we recognize that merely moving to high-dimensional mapping isn't the panacea. It became evident that a marriage of this high-dimensionality with conditions tied to frequency is imperative for enhancing performance. Leveraging these insights, we've constructed a method that samples feature mapping in a manner that meets these specific constraints.

% Consequently, our objective is to devise a more accessible method for feature augmentation in equivariant networks. 
% To achieve this, we establish foundational conditions for feature augmentation compatible with high-dimensional space. 
% However, we found that the high-dimensional mapping is not a sufficient condition, and we need additional conditions related to frequency to make feature augmentation improve performance.
% With these conditions, we develop a method to sample the feature mapping to meet constraints.

% next interest: integration to the neural networks candidates1 - TFN
As we journey forward, the integration of our feature augmentation method into existing equivariant networks takes center stage. Notable architectures like TFN and the SE(3) transformer have paved the way by pioneering the utilization of graph neural network frameworks with the Clebsch-Gordan (CG) product to maintain equivariance. Nevertheless, they do have their Achilles heel – a reliance on the CG product to craft their neural network structure. This dependency becomes a straitjacket, constraining model adaptability.

% With the feature augmentation method, we need to integrate this feature augmentation into equivariant networks. TFN and SE(3) transformer explored the graph neural network architecture with CG product to keep equivariance. However, this method has an architectural bottleneck because it heavily relies on the CG product to build a neural network, which makes the modification of the model hard.

% alternative: Vector Neurons
On the other hand, the Vector Neurons-based equivariant network emerges as a promising alternative. This network, by keeping vectors intact within its neurons and crafting linear and non-linear layers that are in harmony, permits the formation of sequential VN-embedded Multilayered Perceptrons (MLP). What sets this architecture apart is its duality - it integrates effortlessly with renowned point processing networks like PointNet~\cite{qi2017pointnet} and DGCNN~\cite{wang2019dynamic}, and its conceptual framework grounded in elementary linear algebra makes it more digestible.
% In contrast, the Vector Neurons-based equivariant network sidesteps these limitations. By retaining vectors within neurons and devising compatible linear and non-linearity layers, it fosters the creation of sequential VN-embedded Multilayered Perceptrons (MLP). This architecture not only melds seamlessly with prevalent point processing networks like PointNet~\cite{qi2017pointnet} and DGCNN~\cite{wang2019dynamic}, but it's also more intuitively understood due to its foundation in basic linear algebra.

However, Vector Neurons, despite their advantages, are stymied by a constrained feature space. When viewed through the TFN lens, Vector Neurons resemble a TFN derivative, albeit constrained to a 3-dimensional space without the encumbrance of the CG product~\cite{zhu2023e2pn}. However, the breadth of the feature space can be pivotal for performance, so the performance of VN can be limited. 
This limitation manifested in our point completion experiment. As depicted in figure \ref{fig:VN_EVN_recon}, the quality of the reconstructed shapes via VN-OccNet lags behind the OccNet~\cite{mescheder2019occupancy} baseline.

We discovered that the equivariant components used in VN-MLP are not confined to just 3-dimensional vectors but can extend to n-dimensional vectors. By first expanding the dimension of input points from 3 to n before feeding them into VN's layers and maintaining subsequent layers as in VN, we can enhance the intermediate neuron vectors' dimensionality. This approach harnesses the benefits of a high-dimensional feature space, overcoming VN's limitations without compromising its merits.

As a culmination of these findings, we integrated our feature augmentation technique into VN to amplify the dimensionality. In doing so, we effectively combined the strengths of both TFN and VN, while adeptly circumventing their individual pitfalls.

Building upon this foundation, we demonstrate the ease with which our proposed methodology integrates into standard point processing architectures, necessitating only minimal alterations to the existing code. The resulting frameworks, EV-PointNet and EV-DGCNN, stand as testament to our approach's efficacy. Our empirical evaluations underscore the dual advantage of our technique: it not only enforces rotational equivariance but also enhances overall performance across a diverse range of tasks—from shape classification, part segmentation, and normal estimation, to point completion. Notably, infusing our expanded feature methodology into VN culminates in performance metrics that rival—even under canonical orientations—the original model's capabilities. This distinction is especially noteworthy in the realm of equivariant network research, given the common observation that the performance of equivariant structures typically lags behind that of their non-equivariant peers when dealing with aligned datasets. A detailed qualitative analysis further illuminates how our expanded feature dimensions capture the nuanced intricacies of shapes in point completion assignments, as vividly illustrated in figure \ref{fig:VN_EVN_recon}.

Furthermore, we delve into the implications of augmenting feature dimensions in the context of the correspondence-free orientation estimation task, as described by Zhu et al.~\cite{zhu2022correspondence}. This task intrinsically harnesses the equivariance characteristic: when presented with reference and target point clouds of an identical object, the objective becomes pinpointing the relative rotation between the two. As Zhu et al. emphasize, the relative rotation derived within the embedding domain can be coherently mapped to the actual point clouds owing to equivariance. This task not only mandates a holistic, rather than granular, embedding of point clouds while maintaining equivariance but also seeks a superior embedding enriched with details crucial for deducing the relative pose. Our findings resonate with the superiority of our approach: we decidedly eclipse VN benchmarks, which underlines our assertion that dimension expansion facilitates a more refined shape embedding in comparison to traditional VN.

==> method-rotation-v2.tex <==

% **Equivariant Feature Augmentation: Goals and Context**:
Our work seeks to elevate the capabilities of equivariant networks through a specialized feature augmentation strategy. Central to our approach is the development of a base mapping, \(\psi: \mathbb{R}^3 \rightarrow \mathbb{R}^n\), which upholds an intrinsic equivariant relationship. Unlike scalar feature augmentation techniques, like positional embeddings, our method requires an initial definition of a rotation operator in an extended dimensional space. By enhancing multiple foundational mappings \(\psi\), we craft \(\Psi(x)\) — a robust transformation that seamlessly bridges 3D features into their augmented avatars, primed for VN-based networks.


\begin{figure}[t]
\centering
\includegraphics[width=0.99\textwidth]{figure/spherical_revised.png}
\caption{Toy experiment to show the importance of frequency of the augmented features by overfitting networks to reconstruct radial shape functions. The experiment follows the setup of spherical harmonic regression, where the input in points on the sphere $S^2$ and output is magnitude given direction. This will construct the surface by defining continuous magnitude by varying directions. Sequentially from left to right, ground truth shape, reconstructed shape with augmented features of dimension 3, one with repeating 3 twice, one with dimension 3 and 5 but with low frequency, one with dimension 3 and 5 with maximum frequency, and one with dimension 3, 5 and 7 with maximum frequency.}
\label{fig:SH_reg}
\end{figure}

% **Initial Approaches and their Limitations**:
A naive method to instantiate \(\psi\) is simply repeating \(x\) multiple times. Though this approach meets the criteria of equivariance, it introduces redundancy without any subsequent performance gains. This observation crystallized during our experiments centered on radial space mesh reconstruction. Through a neural framework, we mapped the input (a normalized direction) to an augmented feature landscape. We then applied a weighted summation across these features and utilized an MLP for magnitude estimation (see appendix~\ref{app:toy_regression} for the details). However, comparisons between augmentation strategies revealed that a mere duplication of 3D direction data fell short in capturing intricate mesh details as demonstrated in figure \ref{fig:SH_reg}. Therefore, we need a non-trivial method for $\psi$ and we propose such method in the subsequent sections.


\subsection{High-dimensional rotation operator}

Our primary objective is to craft a foundational mapping, \( \psi \), for feature augmentation. To do this effectively, we first need to establish a rotation operator suited for high-dimensional spaces. In this section, we lay out the prerequisites for such rotation operators and then delineate the \( \psi \) mapping that aligns with these rotations. 

For seamless integration with equivariant networks like Vector Neurons~\cite{deng2021vector} and to ensure computational efficiency, we constrain the form of the high-dimensional rotation operator \( D \) to be a matrix within the \( \mathbb{R}^{n \times n} \) space. Consequently, our mapping \( D \) translates from \( SO(3) \) to \( \mathbb{R}^{n \times n} \). For it to function as a high-dimensional rotation operator, we identified specific criteria it must meet, which we refer to as the \textit{rotation's five conditions}.

% \begin{conditions}
% \item A rotation $R \in SO(3)$ should be mapped into a unique $n \times n$ matrix $D(R) \in \mathbb{R}^{n\times n}$ \label{cond:rotationMapping}
% \item \textbf{Identity.} \quad $D(I_{3 \times 3}) = I_{n \times n}$ \label{cond:identity}
% \item \textbf{Injectivity.} \quad $\forall R_1, R_2 \in SO(3), R_1 \neq R_2 \Rightarrow D(R_1) \neq D(R_2)$ \label{cond:injectivity}
% \item \textbf{Compatibility.} \quad $D(R_1R_2)=D(R_1)D(R_2), \quad R_1, R_2 \in SO(3)$ \label{cond:compatibility}
% \item \textbf{Orthonormality.} \quad $D(R)D(R)^T=I_{n \times n}, \quad R \in SO(3)$ \label{cond:orthonormality}
% \end{conditions}

\begin{enumerate}
\item A rotation $R \in SO(3)$ should be mapped into a unique $n \times n$ matrix $D(R) \in \mathbb{R}^{n\times n}$ \label{cond:rotation_1}

\item \textbf{Identity.} \quad
$D(I_{3 \times 3}) = I_{n \times n}$ \label{cond:rotation_2}

\item \textbf{Injectivity.} \quad
$\forall R_1, R_2 \in SO(3), R_1 \neq R_2 \Rightarrow D(R_1) \neq D(R_2) $ \label{cond:rotation_3}

\item \textbf{Compatibility.} \quad
$D(R_1R_2)=D(R_1)D(R_2), \quad R_1, R_2 \in SO(3)$ \label{cond:rotation_4}

\item \textbf{Orthonormality.} \quad
$D(R)D(R)^T=I_{n \times n}, \quad R \in SO(3)$ \label{cond:rotation_5}

\end{enumerate}


% intuitive explanation for each conditions
Each condition is related to the intuition for the rotation. For example, the orthonormality condition is required to preserve magnitude after applying rotation.


\textbf{3-D Rotation Case.}
Before expanding into high-dimensional spaces, understanding the foundational constructs of 3-D rotation is imperative. Specifically, we explore the matrix representation of 3-D rotations, symbolized as \(R \in SO(3)\). Using the axis-angle representation, a rotation matrix is articulated as \(R = \exp(\theta\hat{w}\cdot \vec{F})\), with the unit rotation axis \( \hat{w} \in \mathbb{R}^3 \) (\(|\hat{w}|=1\)), angle \( \theta \in \mathbb{R} \),  $F_1 = \bigl( \begin{smallmatrix}0 & 0 & 0\\ 0 & 0 & -1 \\ 0 & 1 & 0 \end{smallmatrix} \bigr)$, 
$F_2 = \bigl( \begin{smallmatrix}0 & 0 & 1\\ 0 & 0 & 0 \\ -1 & 0 & 0 \end{smallmatrix} \bigr)$, 
$F_3 = \bigl( \begin{smallmatrix}0 & -1 & 0\\ 1 & 0 & 0 \\ 0 & 0 & 0 \end{smallmatrix} \bigr)$, and $\hat{w}\cdot \vec{F}=\sum_{i=1}^3\hat{w}_iF_i$ with $\hat{w}_i$ as i'th element of $\hat{w}$. Intuitively, we can interpret \(\vec{F} = [F_1, F_2, F_3]\) encompasses the matrix bases, with each \(F_i\) being a specific 3x3 matrix, as previously defined.

Our goal of achieving rotation in higher-dimensional space revolves around two pivotal steps: basis generalization in 3-D rotation; expansion to high-dimensional space.

\textbf{Basis Generalization in 3-D Rotation.} Instead of being confined to predetermined matrix bases, we seek to generalize the basis of the rotation matrix \(\vec{F}\). We introduce a condition ensuring that the resulting \(\exp(\theta(\hat{w}\cdot\vec{F}))\) adheres to the properties of a rotation matrix. The criteria for $\vec{F}$ include:
\begin{itemize}
\item \textit{Skew-symmetricity.} This ensures that the resulting matrix is orthonormal. 

\item \textit{Orthogonality of elements.} In matrix terms, this can be expressed as commutative relationships between each pair of basis matrices: \( [F_1, F_2] = F_3 \), \( [F_2, F_3] = F_1 \), and \( [F_3, F_1] = F_2 \). The commutator is represented as \( [A, B] = AB - BA \).

\item \textit{Cyclic property.} It states that rotating by a full cycle using any basis matrix results in the identity matrix, mathematically given by \( \exp(2k\pi F_i) = I_{n \times n} \) for each \( i \in \{1, 2, 3\} \) and for all integers \( k \).
\end{itemize}
We prove that if we can find $\vec{F}$ to meet these three conditions, the $\exp(\theta \hat{w} \cdot \vec{F})$ meets all rotation's five conditions.
This concludes that we can generalize the rotation matrix with different basis $\vec{F}$.



% **3-D Rotation Matrix Basis Generalization.** Rather than using fixed matrix bases, our objective is to expand the rotation matrix basis, \(\vec{F}\). We present the condition, \(\hat{F}\), to guarantee the outcome of \(\exp(\theta(\hat{w}\cdot\vec{F}))\) conforms to rotation matrix properties. The outlined criteria are:
% \begin{itemize}
% \item \textit{Skew-symmetricity:} Guarantees the orthonormality of the resulting matrix.
% \item \textit{Element Orthogonality:} Represented as commutative relations between matrix pairs: \( [F_1, F_2] = F_3 \), \( [F_2, F_3] = F_1 \), \( [F_3, F_1] = F_2 \), with the commutator defined as \( [A, B] = AB - BA \).
% \item \textit{Cyclic Property:} A full rotation using any basis matrix yields the identity matrix: \( \exp(2k\pi F_i) = I_{n \times n} \) for every \( i \in \{1, 2, 3\} \) and integer \( k \).
% \end{itemize}
% By meeting these conditions with \(\vec{F}\), the expression \(\exp(\theta \hat{w} \cdot \vec{F})\) satisfies the essential criteria of a rotation matrix. This indicates the possibility of generalizing the rotation matrix using different basis \(\vec{F}\).

\textbf{Higher Dimensional Generalization.}
Building on the three foundational conditions established for \(\vec{F}\), we now extrapolate to higher dimensions. This initiates the definition of the rotation operator in such spaces:
\begin{equation}
D(R)=\exp(\theta\hat{w}\cdot \vec{\bold{J}})
\label{eq:D}
\end{equation}
Here, \(\theta\) and \(\hat{w}\) denote the angle and axis of $R\in SO(3)$, respectively. \(\vec{\bold{J}}=[J_1, J_2, J_3], J_i \in \mathbb{R}^{n \times n}\) corresponds to the 3-D basis \(\vec{F}\). For \(\vec{J}\), we adopt equivalent conditions from the 3-D case:
\begin{itemize}
\item Each \(J_i\) is both skew-symmetric and distinct: \(J_i^T=-J_i\) and \(J_i \neq 0\) for all \( i \in \{1, 2, 3\}\).
\item Commutation relations: $[J_1,J_2]=J_3, [J_2,J_3]=J_1, [J_3,J_1]=J_2$.
\item The cyclic behavior remains: \(\exp(2k\pi J_i)=I_{n \times n}\) for each \( i \in \{1, 2, 3\}\) and every integer \( k \).
\end{itemize}

\begin{theorem}[properties of $D(R)$]
Given a vector \(\vec{\bold{J}}=[J_1, J_2, J_3], J_i \in \mathbb{R}^{n \times n}\) that satisfies the above conditions, and constructing \(D\) via \(D(R)=\exp(\theta \hat{w}\cdot \vec{\bold{J}})\), where \( \hat{w} \) is the unit rotation axis in \(\mathbb{R}^3\) and \( \theta \) the associated rotation angle in \(\mathbb{R}\) for \(R \in SO(3)\), the matrix \(D\) embodies the following rotation's five conditions.
% \begin{itemize}
%     \item A distinct $n \times n$ matrix $D(R) \in \mathbb{R}^{n\times n}$ represents each rotation $R \in SO(3)$.
%     \item \textbf{Identity:} $D(I_{3 \times 3}) = I_{n \times n}$.
%     \item \textbf{Injectivity:} For all \(R_1, R_2 \in SO(3)\) with \(R_1 \neq R_2\), \(D(R_1) \neq D(R_2) \).
%     \item \textbf{Compatibility:} \(D(R_1R_2)=D(R_1)D(R_2)\) for any \(R_1, R_2 \in SO(3)\).
%     \item \textbf{Orthonormality:} \(D(R)D(R)^T=I_{n \times n}\) for all \( R \in SO(3)\).
% \end{itemize}
\label{thm:D_properties}
\end{theorem}

In essence, if a matrix \(J\) satisfies the three foundational conditions, the resultant \(D\) conforms to the five requirements of a higher-dimensional rotation matrix. The proof is detailed in Appendix~\ref{}. One example for $\vec{J}$ could be derived from three mutually orthogonal vectors:
\begin{equation}
J_1=a_2a_1^\mathsf{T}-a_1a_2^\mathsf{T}, \quad J_2=a_3a_2^\mathsf{T}-a_2a_3^\mathsf{T}, \quad J_3=a_1a_3^\mathsf{T}-a_3a_1^\mathsf{T}
\label{eq:low_frequency_D}
\end{equation}
These vectors $a_1, a_2, a_3\in\mathbb{R}^n$ are constrained by orthogonality and unit norm: \( a_1\cdot a_2=0, a_2\cdot a_3=0, a_3\cdot a_1=0, \ \text{and} \ |a_i|=1 \), and this trivially meets the three condition for $\vec{J}$.

Before delving into the definition of \(\psi\), we present a foundational proposition that serves as a recurring tool throughout this paper.
\begin{proposition}
    Given the rotation \(R\) and the vector \(w\), we have:
    \[(Rw)\cdot\vec{J} = D(R)(w\cdot \vec{J})D(R)^T.\]
\label{prop:axis_rotation}
\end{proposition}
In essence, this proposition suggests that a rotation of the axis in the 3-D space can be translated to a rotation in the n-D space via a similarity transformation employing \(D(R)\), and proof is presented in appendix~\ref{app:}.


% \textbf{Generalization to higher dimensional case.}
% We have extracted three conditions to be $\vec{F}$ to build a rotation matrix. 
% In this section, we will show that these conditions can be generalized to the higher dimensional space. This leads us to define the rotation operator in high-dimensional space as 
% \begin{equation}
% D=\exp(\theta\hat{w}\cdot \vec{\bold{J}})
% \label{eq:D}
% \end{equation}
% where $\theta$ and $\hat{w}$ are angle and axis of $R\in SO(3)$, and $\vec{\bold{J}}=[J_1, J_2, J_3], J_i \in \mathbb{R}^{n \times n}$ corresponding to basis $\vec{F}$ in 3-D cases. And then, we set the same conditions for the $\vec{J}$ as we did for the $\vec{F}$,
% \begin{itemize}
% \item $J_i$ is skew-symmetric and non-zero ($J_i^T=-J_i$, $J_i \neq 0 \text{ for any } i \in \{1, 2, 3\}$)

% \item $[J_1,J_2]=J_3, [J_2,J_3]=J_1, [J_3,J_1]=J_2$ where $[\cdot, \cdot]$ is a commutator ($[A,B]:=AB-BA$)

% \item $\exp(2k\pi J_i)=I_{n \times n} \quad \text{for any } i \in \{1, 2, 3\}, \forall k \in \mathbb{Z}.$
% \end{itemize}

% \begin{theorem}
%     If given $\vec{\bold{J}}=[J_1, J_2, J_3], J_i \in \mathbb{R}^{n \times n}$ satisfies above conditions and $D$ is constructed by $D=\exp(\theta \hat{w}\cdot \vec{\bold{J}})$ where the unit rotation axis \( \hat{w} \in \mathbb{R}^3 \) and angle \( \theta \in \mathbb{R} \) of a rotation $R \in SO(3)$, $D$ satisfies these properties.
%     \begin{itemize}
%     \item A rotation $R \in SO(3)$ should be mapped into a unique $n \times n$ matrix $D(R) \in \mathbb{R}^{n\times n}$
    
%     \item \textbf{Identity.} \quad
%     $D(I_{3 \times 3}) = I_{n \times n}$
    
%     \item \textbf{Injectivity.} \quad
%     $\forall R_1, R_2 \in SO(3), R_1 \neq R_2 \Rightarrow D(R_1) \neq D(R_2) $
    
%     \item \textbf{Compatibility.} \quad
%     $D(R_1R_2)=D(R_1)D(R_2), \quad R_1, R_2 \in SO(3)$
    
%     \item \textbf{Orthonormality.} \quad
%     $D(R)D(R)^T=I_{n \times n}, \quad R \in SO(3)$
    
%     \end{itemize}
%     \label{thm:D_properties}
% \end{theorem}
% Our statement is that if we find $J$ satisfying three conditions, the resultant $D$ satisfies 5 conditions to be a rotation matrix in high-dimensional space. 
% The proof for this Theorem~\ref{thm:D_properties} is in Appendix~\ref{}.




\subsection{Feature Mapping $\psi$ Corresponding to $D$}

To effectively expand our features, we first introduce the rotation operator in the higher-dimensional space. Our goal is to define a mapping $\psi$ for this purpose.

Consider a mapping $\psi: \mathbb{R}^3 \rightarrow \mathbb{R}^n$ that fulfills the rotational equivariance requirement, represented as $\psi(R\vec{x})=D(R)\psi(\vec{x})$, where $\vec{x}$ is any vector from $\mathbb{R}^3$.
{\color{blue} (I need to update this to be more interpretable. Why do we need to assign axis of the rotation to the vector?) The challenge is to identify vectors that align with identical rotations even when situated in diverse dimensional spaces. Our hypothesis is based on the \textit{rotation} concept, which acts as the bridge between the 3-D and n-D spaces. We conjecture that the \textit{axis} of rotation can serve this purpose. Consequently, we introduce the formal definition of the rotation axis in the higher-dimensional space and establish $\psi(x)$ using this concept.}

For an axis to qualify as the base rotation axis, it should remain invariant post rotation with respect to itself. Mathematically, this is represented as $D(R_{\hat{w}}(\theta))v=v$ where $R_{\hat{w}}(\theta)$ is rotation matrix aligned with unit axis $\hat{w}\in \mathbb{R}^3$ by amount of $\theta$. Simplifying further using the condition of $J$, it transforms to $(w\cdot \vec{J})v=0$ where $w=\theta\hat{w}$. Concretly, if $(w\cdot \vec{J})v=0$, then $D(R_{\hat{w}}(\theta))v=\exp(w\cdot \vec{J})v=v$ by definition of matrix exponential. This means that the base axis $v$ is the eigenvector corresponding to the zero eigenvalue of $w\cdot \vec{J}$.

% The conditions to be base axis of the rotation is that the axis should be same after apply rotation with respect to the axis. That is, $D(R_w(\theta))w=w$ where $w\in\mathbb{R}^n$ is base axis in $n$ dimensional space, and $R_w(\theta)\in SO(3)$ is rotation based on $w$ by amount of $\theta$. To make condition simple, we let the condition down to the condition of $J$, and then it becomes $(w\cdot \vec{J})v=0$. Concretly, if $(w\cdot \vec{J})v=0$, then $D(R_w(\theta))v=\exp(\theta w\cdot \vec{J})v=v$ by definition of matrix exponential. That is, base axis $v$ is eigenvector corresponding to zero eigenvalue of $w\cdot \vec{J}$.
\begin{proposition}
    $w\cdot \vec{J}$ has at least one zero eigenvalue.
\label{prop:zero_eig}
\end{proposition}
\begin{proof}
    The proof is in the Appendix.
\end{proof}
The derivation says that we have axis in n-D space for $D(R_w(\theta))$ corresponding to $w$ in 3-D space, and we can obtain that axis by eigenvector of $w\cdot J$ associated to zero eigenvalue, which always exists. Then,
we first define $\psi(x)$ as axis of $D(R_{\hat{x}}(|x|))$, so the $\psi(x)=\{v|(x\cdot\vec{J})v=0\}$. To check equivarant properties, for the every $v$ in $\psi(x)$, $0=D(R)(x\cdot\vec{J})D(R^T)D(R)v=(Rx\cdot\vec{J})D(R)v$ so $D(R)v$ is always eigenvector of $Rx\cdot\vec{J}$ corresponding to zero eigenvalue, which means $D(R)v$ is in $\psi(Rx)$. Therefore, $\psi(x)$ is $SO(3)$ equivariant. 

However, practically there are problems in this definition. We have set of output rather than one determined mapping, so we should choose one vector within the set. Additionally, we should calculate eigen vectors for every $\psi$ calculation, which is computationally inefficient. 

To address these challenges, we leverage the properties of $D$ and propose a practical approach. We first establish an axis in the n-D space that aligns with the $z$-axis in the 3-D space, and then rotate this to align with the axis of $D(R_{\hat{x}}(|x|))$. Formally, if $J_3v=0$ for an eigenvector $v$, the eigenvector of $x\cdot\vec{J}$ can be expressed with $v$ as $D(R^z(\hat{x}))v$.
% Therefore, we convert this into practical form with the property of $D$. The idea is that we first define axis in n-D aligned with $z$ axis in 3-D, and then rotate this to be axis of $D(R_{\hat{x}}(|x|))$. Let's say $v$ is one eigenvector associated with zero eigenvalue (i.e., $J_3v=0$), then we can express eigenvector of $x\cdot\vec{J}$ with $v$ as $D(R^z(\hat{x}))v$, because $(x\cdot\vec{J})D(R^z(\hat{x}))v=D(R^z(\hat{x}))J_3v=0$ by proposition \ref{prop:axis_rotation}. Now, we can define $\psi(x)=D(R^z(\hat{x}))v$ where $J_3v=0$. 
Furthermore, scaling factor does not hurt equivariant properties, so we can introduce tunable scales which have potential to imporove performance, as already introduced as radial function in \cite{Thomas2018TensorFN}. Then, the final form of 
% We introduce our feature mapping function, 
$\psi(\vec{x})$ is as follows.
\begin{equation}
\psi(\vec{x}) = \varphi(|\vec{x}|)D(R^z(\hat{x}))v
\label{eq:feature_mapping}
\end{equation}
In this equation:
\begin{itemize}
    \item $v$ denotes a unit eigenvector of $J_3$ associated with the zero eigenvalue. It's worth noting that any unit vector satisfying $J_3 v = \vec{0}$ can be chosen for $v$, and this choice doesn't influence the equivariance of $\psi(\vec{x})$.
    \item The operation $R^z(\hat{x})$ represents a rotation from the z-axis, given by the vector $[0, 0, 1]$, to $\hat{x}$.
    \item $\varphi: \mathbb{R} \rightarrow \mathbb{R}$ is a function mapping the magnitude of a 3-dimensional feature to a magnitude in a higher-dimensional feature space. Importantly, the specific form of $\varphi$ doesn't affect the equivariance of $\psi(\vec{x})$.
\end{itemize}

\begin{theorem}
\label{thm:psi_equiv}
    $\psi$ satisfies the rotational equivariance $\psi(R\vec{x})=D(R)\psi(\vec{x})$ for any vector $\vec{x} \in \mathbb{R}^3$
\end{theorem}

\begin{proof}
    The proof is in the Appendix.
\end{proof}
It is worth noting that we can generate $v$ before start experiment and keep it during training and test time, which eleminates online calculation of eivenvector.

% where $v$ is a unit eigenvector of $J_3$ corresponding to the zero eigenvalue, operation $R^z(\hat{x})$ is a rotation from z-axis $[0, 0, 1]$ to $\hat{x}$, and $\varphi: \mathbb{R} \rightarrow \mathbb{R}$ is a function mapping from the magnitude of the 3-dimension feature to the magnitude in the high-dimensional feature. This $v$ can be any unit vector that satisfies $J_3 v = \vec{0}$, and the choice of this does not affect the equivariance of $\psi(\vec{x})$. This $\varphi$ can be any function, and it does not affect the equivariance of $\psi(\vec{x})$. 
% % We have tested several design choice of $\varphi$, and simple $\varphi(\vec{x})=|\vec{x}|^{(n-1)/2}$ works best. 
% Then it is proved that the rotational equivariance $\psi(R\vec{x}) = D(R) \psi(\vec{x})$ holds as in \ref{}. Also, if $D$ is fixed, $v$ is unique because the dimension of the null space of $J_3$ is always one. Also, $R^z(\hat{x})$ is unique because a rotation between two vectors is always unique. So, this $\psi(\vec{x})$ is unique given any vector $\vec{x} \in \mathbb{R}^3$.

% \subsection{Importance of frequency}
% % illustrative examples for the representations
% We have a rotation operator in high-dimensional space corresponding to feature mapping for feature augmentation. Now, the problem is that the method to obtain $\vec{J}$. First, we can build $\vec{J}$ from three orthogonal lines as,
% \begin{equation*}
% J_1=a_2a_1^\mathsf{T}-a_1a_2^\mathsf{T}, \quad J_2=a_3a_2^\mathsf{T}-a_2a_3^\mathsf{T}, \quad J_3=a_1a_3^\mathsf{T}-a_3a_1^\mathsf{T}
% \end{equation*}
% where $a_1, a_2, a_3\in\mathbb{R}^n$ is randomly sampled with consraints $\quad a_1\cdot a_2=0,\ a_2\cdot a_3=0,\ a_3\cdot a_1=0, \quad |a_i|=1$. This trivially satisfies three conditions for the $\vec{J}$, so we can build a rotation matrix with \eqref{eq:D} and feature mapping with \eqref{eq:feature_mapping}. However, this method turns out not to increase performance in our toy experiment as shown in figure \ref{fig:SH_reg}. We have to organize what conditions are required for the beneficial feature augmentations.


\subsection{The Role of Frequency in Augmentation}

For feature augmentation, the construct of a rotation operator in high-dimensional spaces provides a roadmap to enhancing feature representation. A pressing challenge emerges in constructing \( \vec{J} \). Initially, we can obtain $\vec{J}$ from \eqref{eq:low_frequency_D}.
% our strategy entailed deriving \( \vec{J} \) from three mutually orthogonal vectors:
% \begin{equation}
% J_1=a_2a_1^\mathsf{T}-a_1a_2^\mathsf{T}, \quad J_2=a_3a_2^\mathsf{T}-a_2a_3^\mathsf{T}, \quad J_3=a_1a_3^\mathsf{T}-a_3a_1^\mathsf{T}
% \label{eq:low_frequency_D}
% \end{equation}
% These vectors $a_1, a_2, a_3\in\mathbb{R}^n$ are constrained by orthogonality and unit norm: \( a_1\cdot a_2=0, a_2\cdot a_3=0, a_3\cdot a_1=0, \ \text{and} \ |a_i|=1 \). 
Although this approach satisfies the foundational requirements for \( \vec{J} \), allowing the formulation of a rotation matrix as per \eqref{eq:D} and a feature map in line with \eqref{eq:feature_mapping}, the empirical outcomes, as evidenced in figure \ref{fig:SH_reg}, don't reflect anticipated improvements. Thus, the spotlight turns to discerning the prerequisites for truly impactful feature augmentations.


% **Gleaning Insights from Previous Works**:
Informed by existing literature, particularly the insights from \cite{tancik2020fourier}, we postulated that truly effective augmented features should possess heightened sensitivity to nuanced input variations, encapsulated by the concept of \textit{frequency}. The essence lies in emphasizing minute input discrepancies, thereby equipping the model to adeptly handle inputs that vary drastically, a characteristic often seen in high-frequency geometries. The act of simple input repetition fails this criterion, as it doesn't bolster the model's ability to discern slight differences. Our overarching ambition, thus, is to forge a \(\psi\) that simultaneously broadens feature dimensionality and intensifies resolution. As we delve deeper in the subsequent sections, our methods, rooted in the intricacies of high-dimensional space rotation, reveal a profound connection: the fidelity of augmented features is intimately linked to the eigenvalues of the encompassing rotation matrix. This insight provides a fresh lens through which the subpar outcomes with \eqref{eq:low_frequency_D} can be understood.

\subsection{Conditions to increase frequency}
Before proceeding, we provide useful propositions for the derivation:
% Throughout the derivation, the following propositions hold:

\begin{proposition}
\label{prop:eigvalue_share}
    Each of $J_1, J_2,$ and $J_3$ shares identical eigenvalues, including both their values and multiplicities.
\end{proposition}

\begin{proposition}
    \label{prop:eigvalue_symmetry}
    \begin{itemize}
        \item The eigenvalues of $J_3$ take the form $\{ -ki, -(k-1)i, \dots, -i, 0, i, \dots, ki\}$ for some non-negative integer $k$
        \item If the absolute values of the eigenvalues are the same, the multiplicities are also the same. That is, if $\lambda$ is an eigenvalue of $J_3$ with multiplicity $m$, then $-\lambda$ is also an eigenvalue of $J_3$ with the same multiplicity $m$.
    \end{itemize}
\end{proposition}


Considering $D=\exp(\theta \hat{w} \cdot \vec{\bold{J}}) = \exp(\theta \bold{J})$, where $\bold{J} = \hat{w} \cdot \vec{\bold{J}}$, the eigenvalues of $\bold{J}$ match those of $J_1, J_2, J_3$ since $\bold{J}$ can be expressed with similariy transform to $J_i$ by the proposition~\ref{prop:axis_rotation}.
% since $J_1, J_2, J_3$ shares the eigenvalues from Proposition~\ref{prop:eigvalue_share}. 
So $\theta \bold{J}$ can be diagonalizable to $\theta \bold{J} = PAP^{-1}$ where $\exists P \in \mathbb{C}^{n \times n}$ is a matrix and $A \in \mathbb{C}^{n \times n}$ is diagonal matrix of the eigenvalues of $\bold{J}$ multiplied by $\theta$, which is $\{ -ki\theta, -(k-1)i\theta, \dots, -i \theta, 0, i\theta, \dots, ki\theta\}$ with their multiplicities.
Then, it is trivial to get $\exp(\theta \bold{J})= \exp(PAP^{-1}) = P \exp(A) P^{-1}$ by using the definition of matrix exponential. 
Also, the matrix exponential of a diagonal matrix is equal to applying scalar exponential elementwise also by using the definition of matrix exponential.
$$\exp\bigl( \begin{smallmatrix}\lambda_1 & \dots & 0\\ \vdots & \ddots & \vdots \\ 0 & \dots & \lambda_n \end{smallmatrix}\bigr) = \bigl( \begin{smallmatrix}\exp(\lambda_1) & \dots & 0\\ \vdots & \ddots & \vdots \\ 0 & \dots & \exp(\lambda_n) \end{smallmatrix}\bigr)$$
So, $D$ can be expressed with 
$$D = \exp(\theta \bold{J}) = \exp(PAP^{-1}) = P \exp(A) P^{-1}
= P \bigl( \begin{smallmatrix}\exp(-ki\theta) & \dots & 0\\ \vdots & \ddots & \vdots \\ 0 & \dots & \exp(ki\theta) \end{smallmatrix}\bigr) P^{-1}$$

\begin{wrapfigure}{r}{0.4\textwidth}
\includegraphics[width=0.99\linewidth]{figure/phi_values_all.png} 
% \caption{Caption1}
% \label{fig:wrapfig}
\end{wrapfigure}
When using our feature mapping from \eqref{eq:feature_mapping} that involves multiplying \( D \) with a vector, each resultant feature element possesses a frequency determined by the maximum value of \( k \). This behavior is visually depicted in the accompanying figures.
To create these figures, we randomly select an axis \( w \) in 3D space and another direction \( x \) orthogonal to \( w \). The figures then depict values of elements in \( \psi(R_w(\theta)x) \), where \( R_w(\theta) \) denotes the rotation matrix with axis \( w \) and angle \( \theta \). Here, \( \theta \) ranges from 0 to 360 degrees. The three plots demonstrate this for maximum \( k \) values of 1, 2, and 3, proceeding from top to bottom. As evidenced by the graphs, the frequency correlates directly with the maximum \( k \), as anticipated.

A compelling observation from the plots is the correlation between the frequency of the resultant feature and the maximum value of $k$. This means that manipulating the value of $k$ in our feature mapping offers a route to control the frequency of the generated augmented features.
\begin{proposition}
    \label{prop:k_bound}
    If $J_3 \in \mathbb{R}^{n \times n}$ and its eigenvalues $\{ -ki, -(k-1)i, \dots, -i, 0, i, \dots, ki\}$ for some non-negative integer $k$ with the multiplicity, the maximum value of $k$ is $\lfloor \frac{n-1}{2} \rfloor$.
\end{proposition}
The highest frequency that this rotation matrix $D$ can handle is now $k \mathbin{/}  2\pi$ from the term $\exp(ki\theta)$ and $\exp(-ki\theta)$. So the frequency of this rotation matrix that can handle is determined by the maximum eigenvalue coefficient $k$. Therefore, we can control the frequency of the base feature $\psi$ by setting eigenvalues of the $J_3$. Given the desired dimension of the feature is $n$, we can set the maximum value of $k = \lfloor \frac{n-1}{2} \rfloor$ by Proposition~\ref{prop:k_bound} to have features with the highest frequency. Through this setting, we can control the frequency of each feature, and then we can construct augmented features by aggregating multiple base features with different frequencies.

% Therefore, any eigenvalue of $D$ takes the form of the exponential of $\theta \lambda$, where $\lambda$ is an eigenvalue of $J_1, J_2, J_3$. From Proposition~\ref{prop:discrete_eigvalue}, the maximum eigenvalue value $n_j$ in each eigenvalue set $\Lambda_j$ corresponds to the frequency that $\Lambda_j$ represents, since the maximum eigenvalue will be $\exp(i n_j \theta)$. Then, the structure of \eqref{eq:feature_mapping} implies that the output features are just linear combinations of $\exp(i n_j \theta)$, and the frequency of this is determined by the maximum frequency ($n_j$). Therefore, we can control the frequency of the base feature $\psi$ by setting eigenvalues of the $J$s.

% Given the base dimension as $n$, we can set the maximum value of $n_j$ to have features with the highest frequency. Through this setting, we can control the frequency of each feature, and then we can construct augmented features by aggregating multiple base features with different frequencies.

% Given this, we can select the optimal combination of $n_j$ values according to their frequencies. We then establish the eigenvalues of $J_1, J_2, J_3$ using the formula $\Lambda_1 + \Lambda_2 + ... + \Lambda_k$, where $\Lambda_j=\{-n_j i, \cdots, -i, 0, i, \cdots, n_j i \}$.

With these eigenvalues set, we can proceed to randomly sample a matrix for $J_3$. Subsequently, the subspaces for $J_1$ and $J_2$ can be reduced using the equations $[J_2, J_3]= J_1$ and $[J_3, J_1]= J_2$. By using cross-entropy method (CEM) optimization with constraint $[J_1, J_2]=J_3$, we determine $J_1$ and $J_2$. Once $J_1, J_2, J_3$ are fixed, $D=\exp(\vec{w} \cdot \vec{\bold{J}})$ can be computed for any given rotation $R \in SO(3)$. Additionally, $\psi(x)$ can be obtained by \eqref{eq:feature_mapping}.

Now we can manipulate the frequency of the base features, which can be utilized to construct feature augmentation. We build a feature by concatenating base feature mapping with dimensions 3 and 5, and the result is much better than previous augmentation methods with \eqref{eq:low_frequency_D} as demonstrated in figure \ref{fig:SH_reg}. The reason for subpar performance of the feature augmentation with \eqref{eq:low_frequency_D} is low frequency due to limited value of $k$, which is 1. This experiment strength our suggestion: not a high-dimensional feature but a high-frequency one matters.

==> method-rotation-v3.tex <==
\section{Effective feature representation with SO(3)-Equivariance}

% **Equivariant feature representation: Goals and Context**:
% Our work seeks to elevate the capabilities of equivariant networks through a specialized feature representation strategy. Central to our approach is the development of a base mapping, \(\psi: \mathbb{R}^3 \rightarrow \mathbb{R}^n\), which upholds an intrinsic equivariant relationship. Unlike scalar feature representation techniques, like positional embeddings, our method requires an initial definition of a rotation operator in an extended dimensional space. By enhancing multiple foundational mappings \(\psi\), we craft \(\Psi(x)\) — a robust transformation that seamlessly bridges 3D features into their augmented avatars, primed for VN-based networks.



% **Initial Approaches and their Limitations**:
% A naive method to instantiate \(\psi\) is simply repeating \(x\) multiple times. Though this approach meets the criteria of equivariance, it introduces redundancy without any subsequent performance gains. This observation crystallized during our experiments centered on radial space mesh reconstruction. Through a neural framework, we mapped the input (a normalized direction) to an augmented feature landscape. We then applied a weighted summation across these features and utilized an MLP for magnitude estimation (see appendix~\ref{app:toy_regression} for the details). However, comparisons between augmentation strategies revealed that a mere duplication of 3D direction data fell short in capturing intricate mesh details as demonstrated in figure \ref{fig:SH_reg}. Therefore, we need a non-trivial method for $\psi$ and we propose such method in the subsequent sections.


\subsection{High-dimensional rotation operator}

% Our primary objective is to determine a mapping, \( \psi \), for feature representation. To do this, we first establish a rotation operator that we will be equivariant with respect to in the feature space. In this section, we lay out the prerequisites for such rotation operators and then delineate the \( \psi \) mapping with respect to those operators. 

% For seamless integration with equivariant networks like Vector Neurons~\cite{deng2021vector} and to ensure computational efficiency, we constrain the form of the high-dimensional rotation operator \( D \) to be a matrix within the \( \mathbb{R}^{n \times n} \) space. 
% In particular, we want $D: SO(3) \rightarrow \mathbb{R}^{n\times n}$ such that it is a high-dimensional rotation operator. We identified specific criteria it must meet, which we refer to as the \textit{rotation's five conditions}.

In this section, we introduce a mapping $D: SO(3) \rightarrow \mathbb{R}^{n \times n}$. A matrix $A \in \mathbb{R}^{n \times n}$ is recognized as a rotation matrix, or part of the special orthogonal group $SO(n)$, if it satisfies the following two conditions:

\begin{itemize}
    \item $AA^T = A^TA = I$: This condition ensures the preservation of the magnitude of the input vector.
    \item $det(A)=1$: This condition ensures the absence of reflective rotation.
\end{itemize}

% However, since we are going to use this mapping $D$ to prove equivariance, we thought it is necessary to satisfy several more conditions. We identified specific criteria it must meet, which we refer to as the conditions (1).
% \paragraph{Conditions (1)}
% \begin{itemize}
% \item All rotation $R \in SO(3)$ should be mapped into one $n \times n$ matrix $D(R) \in \mathbb{R}^{n\times n}$ \label{cond:rotation_1}

% \item \textbf{Identity.} \quad
% $D(I_{3 \times 3}) = I_{n \times n}$ \label{cond:rotation_2}

% \item \textbf{Injectivity.} \quad
% $\forall R_1, R_2 \in SO(3), R_1 \neq R_2 \Rightarrow D(R_1) \neq D(R_2) $ \label{cond:rotation_3}

% \item \textbf{Compatibility.} \quad
% $D(R_1R_2)=D(R_1)D(R_2), \quad R_1, R_2 \in SO(3)$ \label{cond:rotation_4}

% \end{itemize}

% % intuitive explanation for each conditions
% Each condition is related to the intuition for the rotation.
% The uniqueness condition means $D$ is required to be a function from $SO(3)$ to $\mathbb{R}^{n \times n}$.
% The identity condition means that rotating zero angle should not change the feature vector in high-dimension space.
% The injectivity condition means that if a rotation in $SO(3)$ maps the original vector to the different vectors, then $D(R)$ should also map the original one to the different ones.
% The compatibility condition means that the resultant high-dimensional rotation matrix from combining rotations in $SO(3)$ and applying $D$, and applying $D$ to two $R \in SO(3)$ and multiplying are the same.

For the high-dimensional matrix $D(R)$ from the mapping to be considered valid, it must adhere to these two conditions.
However, since the mapping \(D\) is employed to prove the equivariance of the feature representation, it is necessary that it meets several additional conditions, which we term as conditions (1). 

\paragraph{Conditions (1)}
\begin{itemize}
\item All rotations \(R \in SO(3)\) should map to a single \(n \times n\) matrix \(D(R) \in \mathbb{R}^{n\times n}\). \label{cond:rotation_1}

\item \textbf{Identity.} \(D(I_{3 \times 3})\) should equal \(I_{n \times n}\), implying that a zero-angle rotation should not alter the feature vector in high-dimensional space. \label{cond:rotation_2}

\item \textbf{Injectivity.} For any \(R_1, R_2 \in SO(3)\), if \(R_1 \neq R_2\), then \(D(R_1) \neq D(R_2)\). This condition ensures that distinct rotations map to distinct matrices. \label{cond:rotation_3}

\item \textbf{Compatibility.} \(D(R_1R_2)\) should equal \(D(R_1)D(R_2)\) for any \(R_1, R_2 \in SO(3)\), ensuring the resultant high-dimensional rotation matrix remains consistent when combining rotations in \(SO(3)\) and applying \(D\). \label{cond:rotation_4}
\end{itemize}

Each condition is related to the intuition for rotation, ensuring the consistency and uniqueness for ensuring the rotation’s behavior in the high-dimensional space.



\textbf{Exponential form of rotation in 3D.}
We describe the exponential form of $R\in SO(3)$ which we use to derive $D(R)$.
Using the axis-angle representation, a rotation is defined, with the unit rotation axis \( \hat{w} \in \mathbb{R}^3 \) (\(||\hat{w}||=1\)) and angle \( \theta \in \mathbb{R} \). In matrix exponential representation~\cite{hall2013quantum}, a rotation matrix $R$ is expressed as $R=\exp(\theta\hat{w}\cdot\vec{F})$ where $\hat{w}\cdot \vec{F}=\sum_{i=1}^3\hat{w}_iF_i$ with $\hat{w}_i$ as $i^{th}$ element of $\hat{w}$, and $\vec{F} = [F_1, F_2, F_3]$ are pre-defined $ 3 \times 3$ matrices:
\begin{center}
    $F_1 = \begin{bmatrix} \begin{smallmatrix} 0 & 0 & 0 \\ 0 & 0 & -1 \\ 0 & 1 & 0 \end{smallmatrix} \end{bmatrix}$,
    $F_2 = \begin{bmatrix} \begin{smallmatrix} 0 & 0 & 1 \\ 0 & 0 & 0 \\ -1 & 0 & 0 \end{smallmatrix} \end{bmatrix}$,
    $F_3 = \begin{bmatrix} \begin{smallmatrix} 0 & -1 & 0 \\ 1 & 0 & 0 \\ 0 & 0 & 0 \end{smallmatrix} \end{bmatrix}$
\end{center}


% Intuitively, we can interpret \(\vec{F} = [F_1, F_2, F_3]\) encompasses the matrix bases, with each \(F_i\) being a specific 3x3 matrix.
% Intuitively, we can interpret \(\vec{F} = [F_1, F_2, F_3]\), with each \(F_i\) being a specific 3x3 matrix.

% Our goal of achieving rotation in higher-dimensional space revolves around two pivotal steps: basis generalization in 3-D rotation; expansion to high-dimensional space.

% \textbf{Basis Generalization in 3-D Rotation.} Instead of being confined to predetermined matrix bases, we seek to generalize the basis of the rotation matrix \(\vec{F}\). 


% From We introduce general conditions that if $\vec{\bold{J}}=[J_1, J_2, J_3], J_i \in \mathbb{R}^{3 \times 3}$ satisfies then, it adheres to the properties of a rotation matrix stated above. The criteria for $\vec{J}$ include:
% \begin{itemize}
% \item \textit{Skew-symmetricity.} $-J=J^T$. This ensures that the resulting matrix is orthonormal. 

% \item \textit{Commutation relations.} \( [J_1, J_2] = J_3 \), \( [J_2, J_3] = J_1 \), \( [J_3, J_1] = J_2 \) where \( [A, B] = AB - BA \).

% \item \textit{Cyclic property.} \( \exp(2k\pi J_i) = I_{n \times n}, \forall i\in\{\1,2,3\}, \forall k\in \mathbb{Z}\), where $\mathbb{Z}$ denotes the space of integers. 
% % for each \( i \in \{1, 2, 3\} \) and for all integers \( k \).
% \end{itemize}

% \begin{theorem}
%     if $J\in\mathbb{R}^{3\times 3}$ meets the criteria above, then $D(R)=\exp(\theta \hat{w} \cdot \vec{J})$ meets conditions in (1) $\forall R\in SO(3)$.
% \end{theorem}

% We prove that if we can find $\vec{F}$ to meet these three conditions, the $\exp(\theta \hat{w} \cdot \vec{F})$ meets all rotation's five conditions.
% This concludes that we can generalize the rotation matrix with different basis $\vec{F}$.

\textbf{Higher Dimensional Generalization.}
By examining the characteristics of \(\vec{F} = [F_1, F_2, F_3], F_i \in \mathbb{R}^{3 \times 3}\), we identify general conditions for high-dimensional space. If \(\vec{\bold{J}}=[J_1, J_2, J_3], J_i \in \mathbb{R}^{n \times n}\) satisfies these conditions, it complies with the properties of a rotation matrix mentioned above. This insight leads to the definition of the rotation operator in such spaces.
\begin{equation}
D(R)=\exp(\theta\hat{w}\cdot \vec{\bold{J}})
\label{eq:D}
\end{equation}
Here, \(\theta\) and \(\hat{w}\) denote the angle and axis of $R\in SO(3)$, respectively. \(\vec{\bold{J}}=[J_1, J_2, J_3], J_i \in \mathbb{R}^{n \times n}\) corresponds to \(\vec{F} \in \mathbb{R}^{3 \times 3}\). We find the conditions of \(\vec{\bold{J}}\) to satisfy. 

\begin{itemize}
\item \textit{Skew-symmetricity.} $-J=J^T$. This ensures that the resulting matrix is orthonormal. 

\item \textit{Commutation relations.} \( [J_1, J_2] = J_3 \), \( [J_2, J_3] = J_1 \), \( [J_3, J_1] = J_2 \) where \( [A, B] = AB - BA \).

\item \textit{Cyclic property.} \( \exp(2k\pi J_i) = I_{n \times n}, \forall i\in\{\1,2,3\}, \forall k\in \mathbb{Z}\), where $\mathbb{Z}$ denotes the space of integers. 

\end{itemize}

\begin{theorem}
    if $J\in\mathbb{R}^{n\times n}$ meets the criteria above, then $D(R)=\exp(\theta \hat{w} \cdot \vec{J}) \in SO(n)$ and meets conditions in (1) $\forall R\in SO(3)$.
\label{thm:D_properties}
\end{theorem}

In essence, if matrices \(\vec{\bold{J}}\) satisfy these three conditions, the resultant \(D\) conforms to the five requirements of a higher-dimensional rotation matrix. The proof is detailed in Appendix A.

% \begin{theorem}[properties of $D(R)$]
% Given a matrix \(\vec{\bold{J}}=[J_1, J_2, J_3], J_i \in \mathbb{R}^{n \times n}\) that satisfies the above conditions, and constructing \(D\) via \(D(R)=\exp(\theta \hat{w}\cdot \vec{\bold{J}})\), where \( \hat{w} \) is the unit rotation axis in \(\mathbb{R}^3\) and \( \theta \) the associated rotation angle in \(\mathbb{R}\) for \(R \in SO(3)\), the matrix \(D\) embodies the following rotation's five conditions.
% \label{thm:D_properties}
% \end{theorem}

% In essence, if matrices \(\vec{\bold{J}}\) satisfies the three foundational conditions, the resultant \(D\) conforms to the five requirements of a higher-dimensional rotation matrix. The proof is detailed in Appendix~\ref{}. One example for $\vec{\bold{J}}$ could be derived from three mutually orthogonal vectors:
% \begin{equation}
% J_1=a_2a_1^\mathsf{T}-a_1a_2^\mathsf{T}, \quad J_2=a_3a_2^\mathsf{T}-a_2a_3^\mathsf{T}, \quad J_3=a_1a_3^\mathsf{T}-a_3a_1^\mathsf{T}
% \label{eq:low_frequency_D}
% \end{equation}
% These vectors $a_1, a_2, a_3\in\mathbb{R}^n$ are constrained by orthogonality and unit norm: \( a_1\cdot a_2=0, a_2\cdot a_3=0, a_3\cdot a_1=0, \ \text{and} \ |a_i|=1 \), and this trivially meets the three condition for $\vec{\bold{J}}$.

% With these eigenvalues set, we can proceed to randomly sample a matrix for $J_3$. Subsequently, the subspaces for $J_1$ and $J_2$ can be reduced using the equations $[J_2, J_3]= J_1$ and $[J_3, J_1]= J_2$. By using cross-entropy method (CEM) optimization with constraint $[J_1, J_2]=J_3$, we determine $J_1$ and $J_2$. Once $J_1, J_2, J_3$ are fixed, $D=\exp(\vec{w} \cdot \vec{\bold{J}})$ can be computed for any given rotation $R \in SO(3)$. Additionally, $\psi(x)$ can be obtained by \eqref{eq:feature_mapping}.

% {\color{blue} define the alep for determining D(R) here}

% Before delving into the definition of \(\psi\), we present a foundational proposition that serves as a recurring tool throughout this paper.
% \begin{proposition}
%     Given the rotation \(R\in SO(3)\) and the vector \(w\in \mathbb{R}^n\), and $\vec{\bold{J}}=[J_1,J_2,J_3]\in \mathbb{R}^{n \times n}$ defined by theorem \ref{thm:D_properties}, we have:
%     \[(Rw)\cdot\vec{\bold{J}} = D(R)(w\cdot \vec{\bold{J}})D(R)^T.\]
% \label{prop:axis_rotation}
% \end{proposition}
% In essence, this proposition suggests that a rotation of the axis in the 3D space can be translated to a rotation in the n-D space via a similarity transformation employing \(D(R)\), and the proof is presented in appendix~\ref{app:}.


\subsection{feature representation $\psi$ Corresponding to $D$}


In the previous section, we elaborated on the concept of rotation in a high-dimensional space. Now, we provide how to construct an equivariant mapping from \( \mathbb{R}^3 \) to \( \mathbb{R}^n \) using \( D(R) \). This is the mathematical formulation of our mapping:
\begin{equation}
\psi(\vec{x}) = \varphi(||\vec{x}||)D(R^z(\hat{x}))\hat{e}_n.
\label{eq:feature_mapping}
\end{equation}

Wherein:
\begin{itemize}
    \item \( \hat{e}_n \) is a unit eigenvector of \( J_3 \) corresponding to the zero eigenvalue. Notably, the choice of \( \hat{e}_n \) is quite flexible; any unit vector that satisfies \( J_3 \hat{e}_n = \vec{0} \) can serve the purpose without influencing the equivariance of \( \psi(\vec{x}) \).
    \item The term \( R^z(\hat{x}) \) characterizes a rotation from the z-axis (represented by the vector \( \hat{e}_3 = [0, 0, 1] \)) to \( \hat{x} \).
    \item \( \varphi: \mathbb{R} \rightarrow \mathbb{R} \)is a function that scales the magnitude of a three-dimensional vector to a higher-dimensional feature space. The structure of \( \varphi \) does not affect the equivariance of \( \psi(\vec{x}) \).
\end{itemize}

% \begin{theorem}
\begin{restatable}{theorem}{theorempsiequiv}
    The mapping \( \psi \) retains rotational equivariance: \( \psi(R\vec{x})=D(R)\psi(\vec{x}) \) for any vector \( \vec{x} \in \mathbb{R}^3 \).
\label{thm:psi_equiv}
\end{restatable}
% \end{theorem}

The key idea of our methodology is to project a 3D feature onto a high-dimensional space. 
% The conduit for this transformation is uniquely defined by \( D(R) \), given its exclusive accessibility within the nD space.
Conventionally, a point in 3D space can be represented by its magnitude $||\vec{x}||$ and direction $\hat{x} \in \mathbb{R}^3$. This direction $\hat{x}$ can be expressed with a rotation mapping $R^z: \mathbb{R}^3 \rightarrow SO(3)$ from the unit vector of z-axis $\hat{e}_3 = [0, 0, 1]$ to the feature direction $\hat{x}$, denoted by \( R^z(\hat{x}) \). This rotation is unique for each $\hat{x}$ since a rotation between two vectors is unique.  A challenge here is that there is no corresponding z-axis in the high-dimensional space. 

An insight here is that since we know the mapping of the rotation matrix $D: SO(3) \rightarrow \mathbb{R}^{n \times n}$, the z-axis in the higher-dimensional space can be ascertained using a high-dimensional rotation mapped from 3D rotation about the z-axis. The axis-angle representation of 3D rotation about the z-axis is expressed with angle $\theta$ and axis $[0, 0, 1]$, denoted by $R_z(\theta)$, and it cannot change the vector on the z-axis.
Importantly, this derivation holds true even in the high-dimensional space. By the definition of $D(R)$, the high-dimensional rotation matrix corresponding to $R_z(\theta)$ is $D(R)=\exp(\theta J_3)$.


\begin{proposition}
    For a vector \( v\in\mathbb{R}^n \) that satisfies  \( J_3 \hat{e}_n=0 \), then  \( D(R_z(\theta)) \hat{e}_n = \hat{e}_n \), where \( R_z(\theta) \) is a rotation by \( \theta \) about the z-axis.
\end{proposition}

\begin{proposition}
    \( J_3 \) always has zero eigenvalue.
\label{prop:zero_eig}
\end{proposition}

In this approach, the vector \( \hat{e}_n \) in the high-dimensional space, which corresponds to the z-axis in 3D space, is identified using the predefined 
\( D(R) \). This enables us to determine the position of the high-dimensional feature vector $\psi(\vec{x})$ associated with $\vec{x}$ in 3D space by rotating \( D(R^z(\hat{x})) \) from the reference vector \( \hat{e}_n \).

This carefully designed \( \psi(\vec{x}) \) holds the property of equivariance. This is mainly due to its basis on the rotation from a reference vector and the compatibility property of $D(R)$ from the reference vector \( \hat{e}_n \), as in Fig.\ref{fig:psi_equiv}

\begin{figure}[htbp]
\centering
\includegraphics[width=0.5\textwidth]{figure/psi_equiv.png}
\caption{Illustration that shows how $\psi(\hat{x})$ satisfies the equivariance. Features $\hat{x}$ and $R\hat{x}$ are considered as the rotation mapping from the z-axis $\hat{e_3}=[0, 0, 1]$ to the features. Then the relative rotation between them becomes $R$, and the same relationship holds with $D(R)$ in the high-dimensional space $\mathbb{R}^n$.}
\label{fig:psi_equiv}
\end{figure}



% % {\color{red} intuitively explains why rotation-based feature representation would be equivariant}

% % intuitive explanation of feature representation from R^3 to R^n
% Until now, we have defined rotation in the high-dimensional space. As a reminder, our goal is to define a mapping from $\mathbb{R}^3$ to $\mathbb{R}^n$ with equivariance. In this section, we explain how we construct this mapping by utilizing pre-defined $D(R)$ for the rotation in high-dimensional space.

% We first provide the closed form of this mapping, and explain the intuition behind of this. Our mapping is as follows:
% \begin{equation}
% \psi(\vec{x}) = \varphi(||\vec{x}||)D(R^z(\hat{x}))v.
% \label{eq:feature_mapping}
% \end{equation}
% In this equation:
% \begin{itemize}
%     \item $v$ denotes a unit eigenvector of $J_3$ associated with the zero eigenvalue. It's worth noting that any unit vector satisfying $J_3 v = \vec{0}$ can be chosen for $v$, and this choice doesn't influence the equivariance of $\psi(\vec{x})$.
%     \item The operation $R^z(\hat{x})$ represents a rotation from the z-axis, given by the vector $[0, 0, 1]$, to $\hat{x}$.
%     \item $\varphi: \mathbb{R} \rightarrow \mathbb{R}$ is a function mapping the magnitude of a 3-dimensional feature to a magnitude in a higher-dimensional feature space. Importantly, the specific form of $\varphi$ doesn't affect the equivariance of $\psi(\vec{x})$.
% \end{itemize}

% \begin{theorem}
% \label{thm:psi_equiv}
%     $\psi$ satisfies the rotational equivariance $\psi(R\vec{x})=D(R)\psi(\vec{x})$ for any vector $\vec{x} \in \mathbb{R}^3$.
% \end{theorem}

% Our goal is to map a point in 3D space to the one in nD space. Our idea is to define the point in nD space by $D(R)$, because this is the only one we can access for the nD space. We can define a point on the space by magnitude and direction, and direction can be described as rotation from reference axis. That is, direction $\hat{x}\in \mathbb{R}^3$ can be identified by rotating z-axis ($[0,0,1]$) by $R^z(\hat{x})$. However, the problem of this method is we does not have corresponding \textit{z-axis} in the nD space. What we only have in nD space is $D(R)$, so we need to define \textit{z-axis} by rotation.
% We find that we can identify z-axis by applying rotation with respect to z-axis, that is the vector on the z-axis should be invariant to the that rotation. We can convert this condition into the $F_3z=0$, and fortunately, the derivation is also hold in nD space.
% \begin{proposition}
%     If $v\in\mathbb{R}^n$ satisfies $J_3v=0$, then $D(R_z(\theta))v=v$ where $R_z(\theta)$ is rotation by $\theta$ with respect to z-axis.
% \end{proposition}
% \begin{proposition}
%     $J_3$ has at least one zero eigenvalue.
% \label{prop:zero_eig}
% \end{proposition}
% Therefore, we can identify the vector $v$ in nD space corresponding to the z-axis in 3D space by the pre-defined $D(R)$. Now, we have reference axis and the rotation operator in nD space, so we can find the vector in nD space associated with $x$ in 3D space by applying rotation $D(R^z(\hat{x}))$ to the reference frame $v$. 

% This definition of $\psi(x)$ satisfies equivariance property because it can be defined by applying rotation from reference vector and we have competability property of $D(R)$, which make applying addtional rotation equivariant.



% \subsection{Form of $\psi$ to show frequency relation}

% To effectively expand our features, we first introduce the rotation operator in the higher-dimensional space. Our goal is to define a mapping $\psi$ for this purpose.

% Consider a mapping $\psi: \mathbb{R}^3 \rightarrow \mathbb{R}^n$ that fulfills the rotational equivariance requirement, represented as $\psi(R\vec{x})=D(R)\psi(\vec{x})$, where $\vec{x}$ is any vector from $\mathbb{R}^3$.
% {\color{blue} (I need to update this to be more interpretable. Why do we need to assign axis of the rotation to the vector?) The challenge is to identify vectors that align with identical rotations even when situated in diverse dimensional spaces. Our hypothesis is based on the \textit{rotation} concept, which acts as the bridge between the 3-D and n-D spaces. We conjecture that the \textit{axis} of rotation can serve this purpose. Consequently, we introduce the formal definition of the rotation axis in the higher-dimensional space and establish $\psi(x)$ using this concept.}

% For an axis to qualify as the base rotation axis, it should remain invariant post rotation with respect to itself. Mathematically, this is represented as $D(R_{\hat{w}}(\theta))v=v$ where $R_{\hat{w}}(\theta)$ is rotation matrix aligned with unit axis $\hat{w}\in \mathbb{R}^3$ by amount of $\theta$. Simplifying further using the condition of $J$, it transforms to $(w\cdot \vec{J})v=0$ where $w=\theta\hat{w}$. Concretly, if $(w\cdot \vec{J})v=0$, then $D(R_{\hat{w}}(\theta))v=\exp(w\cdot \vec{J})v=v$ by definition of matrix exponential. This means that the base axis $v$ is the eigenvector corresponding to the zero eigenvalue of $w\cdot \vec{J}$.

% \begin{proposition}
%     $w\cdot \vec{J}$ has at least one zero eigenvalue.
% \label{prop:zero_eig}
% \end{proposition}
% \begin{proof}
%     The proof is in the Appendix.
% \end{proof}
% The derivation says that we have axis in n-D space for $D(R_w(\theta))$ corresponding to $w$ in 3-D space, and we can obtain that axis by eigenvector of $w\cdot J$ associated to zero eigenvalue, which always exists. Then,
% we first define $\psi(x)$ as axis of $D(R_{\hat{x}}(|x|))$, so the $\psi(x)=\{v|(x\cdot\vec{J})v=0\}$. To check equivarant properties, for the every $v$ in $\psi(x)$, $0=D(R)(x\cdot\vec{J})D(R^T)D(R)v=(Rx\cdot\vec{J})D(R)v$ so $D(R)v$ is always eigenvector of $Rx\cdot\vec{J}$ corresponding to zero eigenvalue, which means $D(R)v$ is in $\psi(Rx)$. Therefore, $\psi(x)$ is $SO(3)$ equivariant. 

% However, practically there are problems in this definition. We have set of output rather than one determined mapping, so we should choose one vector within the set. Additionally, we should calculate eigen vectors for every $\psi$ calculation, which is computationally inefficient. 

% To address these challenges, we leverage the properties of $D$ and propose a practical approach. We first establish an axis in the n-D space that aligns with the $z$-axis in the 3-D space, and then rotate this to align with the axis of $D(R_{\hat{x}}(|x|))$. Formally, if $J_3v=0$ for an eigenvector $v$, the eigenvector of $x\cdot\vec{J}$ can be expressed with $v$ as $D(R^z(\hat{x}))v$.
% % Therefore, we convert this into practical form with the property of $D$. The idea is that we first define axis in n-D aligned with $z$ axis in 3-D, and then rotate this to be axis of $D(R_{\hat{x}}(|x|))$. Let's say $v$ is one eigenvector associated with zero eigenvalue (i.e., $J_3v=0$), then we can express eigenvector of $x\cdot\vec{J}$ with $v$ as $D(R^z(\hat{x}))v$, because $(x\cdot\vec{J})D(R^z(\hat{x}))v=D(R^z(\hat{x}))J_3v=0$ by proposition \ref{prop:axis_rotation}. Now, we can define $\psi(x)=D(R^z(\hat{x}))v$ where $J_3v=0$. 
% Furthermore, scaling factor does not hurt equivariant properties, so we can introduce tunable scales which have potential to imporove performance, as already introduced as radial function in \cite{Thomas2018TensorFN}. Then, the final form of 
% % We introduce our feature representation function, 
% $\psi(\vec{x})$ is as follows.
% \begin{equation}
% \psi(\vec{x}) = \varphi(||\vec{x}||)D(R^z(\hat{x}))v
% \label{eq:feature_mapping}
% \end{equation}
% In this equation:
% \begin{itemize}
%     \item $v$ denotes a unit eigenvector of $J_3$ associated with the zero eigenvalue. It's worth noting that any unit vector satisfying $J_3 v = \vec{0}$ can be chosen for $v$, and this choice doesn't influence the equivariance of $\psi(\vec{x})$.
%     \item The operation $R^z(\hat{x})$ represents a rotation from the z-axis, given by the vector $[0, 0, 1]$, to $\hat{x}$.
%     \item $\varphi: \mathbb{R} \rightarrow \mathbb{R}$ is a function mapping the magnitude of a 3-dimensional feature to a magnitude in a higher-dimensional feature space. Importantly, the specific form of $\varphi$ doesn't affect the equivariance of $\psi(\vec{x})$.
% \end{itemize}

% \begin{theorem}
% \label{thm:psi_equiv}
%     $\psi$ satisfies the rotational equivariance $\psi(R\vec{x})=D(R)\psi(\vec{x})$ for any vector $\vec{x} \in \mathbb{R}^3$
% \end{theorem}

% \begin{proof}
%     The proof is in the Appendix.
% \end{proof}
% It is worth noting that we can generate $v$ before start experiment and keep it during training and test time, which eleminates online calculation of eivenvector.


\subsection{The Role of Frequency in Augmentation}

% {\color{blue}
% explain you need to turn inputs to be on a unit sphere

% explain how each point can be determined using angle on sphere

% express $\psi(x)$ in sinusoids

% explain what it means to have high frequency in sinusoids of $\psi(x)$

% explain how the eigenvalues of $D(R)$ impacts the frequency, and how you can attain high frequency $\psi(x)$

% }

% \subsection{Conditions to increase frequency}
Before proceeding, we provide useful propositions for the derivation:

\begin{proposition}
\label{prop:eigvalue_share}
    Each of $J_1, J_2,$ and $J_3$ shares all eigenvalues, and multiplicities.
\end{proposition}

\begin{proposition}
    \label{prop:eigvalue_symmetry}
    The eigenvalues of $J_3$ satisfy these two conditions.
    \begin{itemize}
        \item The eigenvalues of $J_3$ take the form $\{ -ki, -(k-1)i, \dots, -i, 0, i, \dots, ki\}$ for some non-negative integer $k$
        \item If $\lambda$ is an eigenvalue of $J_3$ with multiplicity $m$, then $-\lambda$ is also an eigenvalue of $J_3$ with the same multiplicity $m$.
    \end{itemize}
\end{proposition}

\begin{proposition}
    % Given the rotation \(R\) and the vector \(w\), we have:
    % \[(Rw)\cdot\vec{J} = D(R)(w\cdot \vec{J})D(R)^T.\]
    Given a unit vector $\hat{w} \in \mathbb{R}^3$, 
    $$\hat{w} \cdot \vec{\bold{J}} = D(R)J_3D(R)^T$$
    where $R$ is a rotation mapping from $[0, 0, 1]$ to $\hat{w}$
\label{prop:axis_rotation}
\end{proposition}


Considering $D(R)=\exp(\theta \hat{w} \cdot \vec{\bold{J}}) = \exp(\theta \bold{J})$, where $\bold{J} = \hat{w} \cdot \vec{\bold{J}}$, the eigenvalues of $\bold{J}$ match those of $J_1, J_2, J_3$ since $\bold{J}$ can be expressed with similariy transform to $J_i$ by the proposition~\ref{prop:axis_rotation}.
% since $J_1, J_2, J_3$ shares the eigenvalues from Proposition~\ref{prop:eigvalue_share}. 
So $\theta \bold{J}$ can be diagonalizable to $\theta \bold{J} = PAP^{-1}$ where $ P \in \mathbb{C}^{n \times n}$ is a matrix and $A \in \mathbb{C}^{n \times n}$ is diagonal matrix of the eigenvalues of $\bold{J}$ multiplied by $\theta$, which is $\{ -ki\theta, -(k-1)i\theta, \dots, -i \theta, 0, i\theta, \dots, ki\theta\}$ with their multiplicities.
From the definition of the matrix exponential, it is trivial to get $\exp(\theta \bold{J})= \exp(PAP^{-1}) = P \exp(A) P^{-1}$ and 
\begin{equation*}
\exp \begin{bsmallmatrix}\lambda_1 & \dots & 0\\ \vdots & \ddots & \vdots \\ 0 & \dots & \lambda_n \end{bsmallmatrix} =  \begin{bsmallmatrix}\exp(\lambda_1) & \dots & 0\\ \vdots & \ddots & \vdots \\ 0 & \dots & \exp(\lambda_n) \end{bsmallmatrix}
\end{equation*}
So, $D(R)$ can be expressed with 
\begin{equation*}
D(R)
= P\begin{bsmallmatrix}\exp(-ki\theta) & \dots & 0\\ \vdots & \ddots & \vdots \\ 0 & \dots & \exp(ki\theta) \end{bsmallmatrix} P^{-1}
= P\begin{bsmallmatrix}\cos(-k\theta)+i\sin(-k\theta) & \dots & 0\\ \vdots & \ddots & \vdots \\ 0 & \dots & \cos(k\theta)+i\sin(k\theta) \end{bsmallmatrix} P^{-1}
\end{equation*}

% \begin{wrapfigure}{r}{0.4\textwidth}
% \includegraphics[width=0.99\linewidth]{figure/phi_values_all.png} 
% % \caption{Caption1}
% % \label{fig:wrapfig}
% \end{wrapfigure}
% When using our feature representation from \eqref{eq:feature_mapping} that involves multiplying \( D \) with a vector, each resultant feature element possesses a frequency determined by the maximum value of \( k \). This behavior is visually depicted in the accompanying figures.
% To create these figures, we randomly select an axis \( w \) in 3D space and another direction \( x \) orthogonal to \( w \). The figures then depict values of elements in \( \psi(R_w(\theta)x) \), where \( R_w(\theta) \) denotes the rotation matrix with axis \( w \) and angle \( \theta \). Here, \( \theta \) ranges from 0 to 360 degrees. The three plots demonstrate this for maximum \( k \) values of 1, 2, and 3, proceeding from top to bottom. As evidenced by the graphs, the frequency correlates directly with the maximum \( k \), as anticipated.

A compelling observation is the correlation between the frequency of the resultant feature and the magnitude of $k$. This means that manipulating the value of $k$ in our feature representation offers a route to control the frequency of the generated augmented features.
\begin{proposition}
    \label{prop:k_bound}
    If $J_3 \in \mathbb{R}^{n \times n}$ and its eigenvalues $\{ -ki, -(k-1)i, \dots, -i, 0, i, \dots, ki\}$ for some non-negative integer $k$ with the multiplicity, the maximum value of $k$ is $\lfloor \frac{n-1}{2} \rfloor$.
\end{proposition}
The highest frequency that this rotation matrix $D$ can handle is now $k \mathbin{/}  2\pi$ from the term $\cos(\pm k\theta)$ and $\sin(\pm k\theta)$. So the frequency of this rotation matrix that can handle is determined by the maximum eigenvalue coefficient $k$. Therefore, we can control the frequency of the base feature $\psi$ by setting eigenvalues of the $J_3$. Given the desired dimension of the feature is $n$, we can set the maximum value of $k = \lfloor \frac{n-1}{2} \rfloor$ by Proposition~\ref{prop:k_bound} to have features with the highest frequency. Through this setting, we can control the frequency of each feature, and then we can construct augmented features by aggregating multiple base features with different frequencies.

\begin{figure}[tbp]
\centering
\includegraphics[width=0.99\textwidth]{figure/spherical_revised.png}
\caption{ Toy experiment to show the importance of frequency of the augmented features by overfitting networks to reconstruct radial shape functions. The experiment follows the setup of spherical harmonic regression, where the input in points on the sphere $S^2$ and output is magnitude given direction. This will construct the surface by defining continuous magnitude by varying directions. Sequentially from left to right, ground truth shape, reconstructed shape with augmented features of dimension 3, one with repeating 3 twice, one with dimension 3 and 5 but with low frequency, one with dimension 3 and 5 with maximum frequency, and one with dimension 3, 5 and 7 with maximum frequency.}
\label{fig:SH_reg}
\end{figure}

% Now we can manipulate the frequency of the base features, which can be utilized to construct feature representation. We build a feature by concatenating base feature representation with dimensions 3 and 5, and the result is much better than previous augmentation methods with \eqref{eq:low_frequency_D} as demonstrated in figure \ref{fig:SH_reg}. The reason for the subpar performance of the feature representation with \eqref{eq:low_frequency_D} is low frequency due to the limited value of $k$, which is 1. This experiment strengthens our suggestion: not a high-dimensional feature but a high-frequency one matters.

Additionally, we can convert $\psi$ into a sinusoidal formulation which reveals an important relation between frequency and eigenvalues. Then, the rotation angle $\theta$ and axis $\vec{w}$ of the rotation $R^z(\hat{x})$ depend on $\vec{x}$. From Section 4.3, 

\begin{equation*}
D(R^z(\hat{x})) = \exp(\vec{w} \cdot \vec{\bold{J}})
= P \bold{\Lambda} P^{-1}
= \sum_{i=1}^{n} \vec{b}_i{\vec{b}_i}^T(\sin(k_i\theta)+\mathrm{i}\cos(k_i\theta))
\end{equation*}

where $\bold{\Lambda} \in \mathbb{C}^{n \times n}$ is the diagonal matrix whose diagonal elements are $\bold{\Lambda}_{ii} = \sin(k_i\theta)+\mathrm{i}\cos(k_i\theta)$. $P\in \mathbb{C}^{n \times n}$  whose $i^{th}$ column is the eigenvector $\vec{b}_i$ of $\vec{w} \cdot \vec{\bold{J}}$. Then $\psi(\vec{x})$ can be described with a sinusoidal function of $\theta$.


\begin{align}
\psi(\vec{x}) & = \varphi(||\vec{x}||)D(R^z(\hat{x})) \hat{e}_n \\
& = \varphi(||\vec{x}||) \sum_i \vec{b}_i {\vec{b}_i}^T(\sin(k_i\theta)+\mathrm{i}\cos(k_i\theta)) \hat{e}_n \\
& = \varphi(||\vec{x}||) \sum_i (\vec{b}_i\cdot \hat{e}_n) (\sin(k_i\theta)+\mathrm{i}\cos(k_i\theta)) \vec{b}_i
% \psi(x) & =aD(R)v=a\sum_ib_ib_i^T(\sin(k_i\theta)+\mathrm{i}\cos(k_i\theta))v=\sum_ia(b_i\cdot v)(\sin(k_i\theta)+\mathrm{i}\cos(k_i\theta))b_i
\label{eq:psi_sinusoidal}
\end{align}

where $a\in\mathbb{R}$ is scale factor, $b_i$ is eigenvector of $J_3$ associated with the eigenvalue of $k_i\mathrm{i}$.

{\color{blue} explain how spherical harmonic can be discovered this way}

We observe how the frequency in the augmented feature is depicted by the eigenvalues of \(J_i\). Assuming that utilizing only three dimensions does not adequately capture the shape details, we opt for the addition of 5-dimensional features. From Proposition~\ref{prop:k_bound}, the eigenvalues including multiplicity will be either \(\Lambda_1 = \{-\mathrm{i}, 0, 0, 0, \mathrm{i}\}\) or \(\Lambda_2 = \{-2\mathrm{i}, -\mathrm{i}, 0, \mathrm{i}, 2\mathrm{i}\}\). Based on \eqref{eq:psi_sinusoidal}, higher magnitude eigenvalues render \(\psi\) more sensitive to the input feature, thereby capturing more details. Fig.~\ref{fig:SH_reg} demonstrates the impact of the frequency of the augmented feature on the shape details. A low frequency, where the 5-dimensional augmented feature used \(J_3\) with eigenvalues of \(\Lambda_1\), shows negligible improvement. However, employing the maximum frequency, with the augmented feature using \(J_3\) having eigenvalues of \(\Lambda_2\), results in a significant enhancement compared to the low-frequency augmented feature.


\subsection{Obtaining Impactful Feature Agumentation}

What we want here is to get feature representation with multiple frequencies, governed by the dimension of the feature $n$. We construct concatenated feature representation $\Psi(x)$ by concatenating representation with sequentially increasing frequency as $\Psi(x)=\oplus_{k=1}^{r}\psi(x;k)$ where $\psi(x;k)$ indicate $\psi$ constructed by set of eigenvalues $[-k\mathrm{i}, \cdots, k\mathrm{i}]$ in $\vec{J}$ as described in proposition \ref{prop:k_bound}.
With this technique, we can effectively express multiple frequency features for the 3D data, which eventually enables the model to describe further details to get higher performance.

Finally, we present pseudo code for sampling $J_1, J_2$, and $J_3$ with the desired frequency. This will build $D(R)$ followed by $\psi(x)$ for the proposed feature representation technique.

\begin{minipage}[t]{0.48\textwidth}
\begin{algorithm}[H]
\caption{Sample $J_1, J_2, J_3$}
\begin{algorithmic}[1]
\Require $n$
\State $J_3 \gets \text{\textsc{Sample}}J_3(n)$
\State find bases of constraints in Equation~\ref{eq:J123_linear_condition}
% \State $J_1, J_2 \gets \text{\textsc{Optimize}}J_1, J_2(n, J_3)$
\State $J_1, J_2 \gets \text{CEM with loss }\lVert J_1J_2-J_2J_1-J_3 \rVert_F^2$
\State \Return $[J_1, J_2, J_3]$
\end{algorithmic}
\label{alg:sample_Js}
\end{algorithm}
\end{minipage}
\hfill
\begin{minipage}[t]{0.48\textwidth}
\begin{algorithm}[H]
\caption{\textsc{Sample}$J_3$}
\begin{algorithmic}[1]
\Require $n$
\State $A \gets$ randomly fill $\mathbb{R}^{n\times n}$ matrix
\State $J_3 \gets A - A^T$
\State $U \gets \textsc{GetEigenVectors}(J_3)$
\State $\Lambda = \text{\textsc{diagonal}}([-\lfloor\frac{n-1}{2}\rfloor \mathrm{i}, \dots, \lfloor\frac{n-1}{2}\rfloor \mathrm{i}])$
\State $J_3 \gets U\Lambda U^*$
\State \Return $J_3$
\end{algorithmic}
\label{alg:sample_J3}
\end{algorithm}
\end{minipage}%

First, we pick \( J_3 \). The exact choice between \( J_3 \), \( J_1 \), or \( J_2 \) isn't crucial since \( \psi \) will remain equivariant regardless. To get \( J_3 \), we start with a random skew-symmetric matrix. We then adjust its eigenvalues to \( [-\lfloor \frac{n-1}{2}\mathrm{i} \rfloor, \dots, \lfloor \frac{n-1}{2}\mathrm{i} \rfloor] \) while keeping the eigenvectors unchanged. 

Our next task is to figure out \( J_1 \) and \( J_2 \), bearing in mind the conditions mentioned in Theorem \ref{thm:D_properties}. From these conditions, we can pinpoint four key rules:
\begin{equation}
\textsc{diag}(J_1)=0, \textsc{diag}(J_2)=0, [J_3,J_1]=J_2, [J_2,J_3]=J_1
\label{eq:J123_linear_condition}
\end{equation}
where $\textsc{diag}(X)$ is diagonal components of squared matrix $X$.
These rules can be reshaped into a linear format: \( A[\textsc{vec}(J_1), \textsc{vec}(J_2)]^T=0 \), where \( \textsc{vec}(\cdot) \) is the process of turning it into a vector. The nullspace of \( A \) gives us the foundational elements for \( [J_1, J_2] \). Potential \( J_1 \) and \( J_2 \) values can be depicted as combinations of these elements.

Next, we search the space made by the base elements of \( [J_1, J_2] \) using the Cross Entropy Method (CEM)~\cite{de2005tutorial}. We measure the accuracy using the loss \( \lVert J_1J_2-J_2J_1-J_3 \rVert_F^2 \), where \( \lVert \cdot \rVert_F \) is the Frobenius norm. At the end of this process, we have our \( [J_1, J_2, J_3] \) values, which enables us to build both \( D(R) \) and \( \psi(x) \).

==> method-rotation.tex <==

In this section, we aim to develop a mapping $\phi: \mathbb{R}^3 \rightarrow \mathbb{R}^n$ which is utilized to feature augmentation in the equivariant networks.

One naive idea to realize $\phi$ is repeating $x$ several times. (i.g., $\phi(x)=x\oplus x$ where $\oplus$ means concatenation). This $\psi$ is equivariant because $\phi(Rx)=D(R)\phi(x)$ where $D(R)=R\oplus R$. However, this makes the feature redundant and we find that performance is not increased in our experiment (section \ref{Experiment}).
Inspired by \cite{tancik2020fourier}, the useful features to be augmented are more sensitive to the small difference in the input, which is related to the frequency. That is the augmented features amplify small differences in input, which makes the model able to handle aggressively changed inputs (i.e., high-frequency geometry in the shapes). In this perspective, repeating input is not useful because it does not increase the capability to capture smaller differences. Therefore, our goal is to develop a $\phi$ which can increase feature dimension while increasing the resolution of the features. In this section, we propose such a method starting from defining rotation in high dimensional space. In the end, we reveal that the resolution of the augmented feature is highly related to the eigenvalues of the rotation matrix in high dimensional space.

% Our research aims to achieve the rotation of a feature vector within a high-dimensional space, all while ensuring rotational equivariance. 
% To achieve this, two essential components must be established. 
% Firstly, a high-dimensional rotation operator should be defined to ensure the desired rotational transformations can be applied consistently. 
% Additionally, considering that most of the shape data is given by a 3D point cloud, a mapping function that can transform from 3D data into a high-dimensional space while preserving rotation equivariance is required. 

\subsection{High-dimensional rotation operator}

To be compatible with the Vector Neurons' layers and computational efficiency, we limit the form of the high-dimensional rotation operator $D$ as a matrix in $\mathbb{R}^{n \times n}$ space.
Here we define a mapping $D$ from $SO(3)$ to $\mathbb{R}^{n \times n}$.
To be a high-dimensional rotation operator, we find out that it should satisfy these conditions.

\begin{itemize}
\item A rotation $R \in SO(3)$ should be mapped into a unique $n \times n$ matrix $D(R) \in \mathbb{R}^{n\times n}$

\item Identity
$$D(I_{3 \times 3}) = I_{n \times n}$$

\item Injectivity 
$$\forall R_1, R_2 \in SO(3), R_1 \neq R_2 \Rightarrow D(R_1) \neq D(R_2) $$

\item Compatibility 
$$D(R_1R_2)=D(R_1)D(R_2), \quad R_1, R_2 \in SO(3)$$

\item Orthonormality
$$D(R)D(R)^T=I_{n \times n}, \quad R \in SO(3)$$

\end{itemize}

Our proposed high-dimensional rotation operator $D$ is defined as below, and it is proved that this $D$ satisfies the four necessary conditions above.

$$D=\exp(\vec{w} \cdot \vec{\bold{J}})$$
$$\text{where }\vec{w} \text{ is the axis-angle representation of }R \in SO(3)$$
$$\vec{\bold{J}}=[J_1, J_2, J_3], J_i \in \mathbb{R}^{n \times n}$$

This matrix set $\{J_1, J_2, J_3\} \in \mathbb{R}^{n\times n}$  should satisfy below conditions.
\begin{itemize}
\item $J_i$ is skew-symmetric and non-zero ($J_i^T=-J_i$, $J_i \neq 0 \text{ for any } i \in \{1, 2, 3\}$)

\item $[J_1,J_2]=J_3, [J_2,J_3]=J_1, [J_3,J_1]=J_2$ where $[\cdot, \cdot]$ is a commutator ($[A,B]:=AB-BA$)

\item $\exp(2k\pi J_i)=I_{n \times n} \quad \text{for any } i \in \{1, 2, 3\}, \forall k \in \mathbb{Z}$

% \item One of $J_i$ should have $n$ distinct eigenvalues.

\end{itemize}

% intuition behind this design
The intuition behind this design choice is, $F_1 = \bigl( \begin{smallmatrix}0 & 0 & 0\\ 0 & 0 & -1 \\ 0 & 1 & 0 \end{smallmatrix} \bigr)$, 
$F_2 = \bigl( \begin{smallmatrix}0 & 0 & 1\\ 0 & 0 & 0 \\ -1 & 0 & 0 \end{smallmatrix} \bigr)$, 
$F_3 = \bigl( \begin{smallmatrix}0 & -1 & 0\\ 1 & 0 & 0 \\ 0 & 0 & 0 \end{smallmatrix} \bigr)$ always satisfy $R=\exp(\vec{w} \cdot \vec{\bold{F}})$ given any rotation $R \in SO(3)$, and $F_1, F_2, F_3$ satisfy the conditions on $J_1, J_2, J_3$ when $n=3$.

Based on the definition of $D(R)$ and $J_1, J_2, J_3$, we derived five necessary conditions for a high-dimensional rotation operation. Detailed proofs for these are provided in the appendix. Throughout the derivation, the following propositions hold:

\begin{proposition}
\label{prop:eigval_share}
    Each of $J_1, J_2,$ and $J_3$ shares identical eigenvalues, including both their values and multiplicities.
\end{proposition}

\begin{proposition}
    \label{prop:discrete_eigvalue}
    Let $\Lambda_j=\{-n_j i, \cdots, -i, 0, i, \cdots, n_j i \}$ where $n_j \geq 0$ and $n_j \in \mathbb{Z}$ represent the set of consecutive eigenvalues. The eigenvalues of $J_1, J_2, J_3 \in \mathbb{R}^{n \times n}$  should then be the combined set of these eigenvalues with their respective multiplicities, formulated as: $\Lambda_1 + \Lambda_2 + ... + \Lambda_k$
\end{proposition}

Considering $D=\exp(\vec{w} \cdot \vec{\bold{J}}) = \exp(\theta \bold{J})$, where $\theta = ||\vec{w}||, \bold{J} = \hat{w} \cdot \vec{\bold{J}}$, the eigenvalues of $\bold{J}$ match those of $J_1, J_2, J_3$. Therefore, any eigenvalue of $D$ takes the form of the exponential of $\theta \lambda$, where $\lambda$ is an eigenvalue of $J_1, J_2, J_3$. From Proposition~\ref{prop:discrete_eigvalue}, the maximum eigenvalue value $n_j$ in each eigenvalue set $\Lambda_j$ corresponds to the frequency that $\Lambda_j$ represents, since the maximum eigenvalue will be $\exp(i n_j \theta)$. 

Given this, we can select the optimal combination of $n_j$ values according to their frequencies. We then establish the eigenvalues of $J_1, J_2, J_3$ using the formula $\Lambda_1 + \Lambda_2 + ... + \Lambda_k$, where $\Lambda_j=\{-n_j i, \cdots, -i, 0, i, \cdots, n_j i \}$.

With these eigenvalues set, we can proceed to randomly sample a matrix for $J_3$. Subsequently, the subspaces for $J_1$ and $J_2$ can be reduced using the equations $[J_2, J_3]= J_1$ and $[J_3, J_1]= J_2$. By using cross-entropy method (CEM) optimization with constraint $[J_1, J_2]=J_3$, we determine $J_1$ and $J_2$. Once $J_1, J_2, J_3$ are fixed, $D=\exp(\vec{w} \cdot \vec{\bold{J}})$ can be computed for any given rotation $R \in SO(3)$.


\subsection{Equivariant transform from 3D into a high-dimensional space}

The next essential mapping is to transform from 3D data into a high-dimensional space while preserving rotation equivariance. We define a mapping $\psi:\mathbb{R}^3 \rightarrow \mathbb{R}^n$, and it should satisfy the rotational equivariance $\psi(R\vec{x})=D(R)\psi(\vec{x})$ for any vector $\vec{x} \in \mathbb{R}^3$.

We propose our $\psi(\vec{x})$ as below.

$$\psi(\vec{x}) = \varphi(|\vec{x}|)D(R^z(\hat{x}))v$$

where $v$ is a unit eigenvector of $J_3$ corresponding to the zero eigenvalue, operation $R^z(\hat{x})$ is a rotation from z-axis $[0, 0, 1]$ to $\hat{x}$, and $\varphi: \mathbb{R} \rightarrow \mathbb{R}$ is arbitrary mapping from magnitude of the vector to the magnitude in the high dimensional feature space. We have tested several design choice of $\varphi$, and simple $\varphi(\vec{x})=|\vec{x}|^{(n-1)/2}$ works best. Then it is proved that the rotational equivariance $\psi(R\vec{x}) = D(R) \psi(\vec{x})$ holds. Also, if $D$ is fixed, $v$ is unique because the dimension of the null space of $J_3$ is always one. Also, $R^z(\hat{x})$ is unique because a rotation between two vectors is always unique. So, this $\psi(\vec{x})$ is unique given any vector $\vec{x} \in \mathbb{R}^3$.


\begin{figure}[t]
\centering
\includegraphics[width=0.97\textwidth]{figure/spherical_regression.png}
\caption{Toy experiment to show the importance of frequency of the augmented features by overfitting networks to reconstruct radial shape functions. The experiment follows the setup of spherical harmonic regression, where the input in points on the sphere $S^2$ and output is magnitude given direction. This will construct the surface by defining continuous magnitude by varying directions. Sequentially from left to right, ground truth shape, reconstructed shape with augmented features of dimension 3, one with repeating 3 twice, one with dimension 3 and 5, and finally one with dimension 3, 5, and 7.}
\label{fig:SH_reg}
\end{figure}


==> preliminaries.tex <==
\section{Problem Setting}

% \subsection{Vector Neurons}
% \cite{deng2021vector} introduced the Vector Neurons approach to embed rotational equivariance into conventional neural networks. This is achieved by ensuring $SO(3)$ equivariance through a three-step process. Initially, a permutation invariant dimension is generated via edge convolution using a given point cloud. When the point cloud's dimension is $N \times 3$, an additional permutation invariant feature dimension $C$ is introduced, resulting in a dimension of $N \times C \times 3$. Subsequently, rotation equivariant layers act on the $F$ dimension, ensuring the feature retains its $3$ dimension while conforming to $SO(3)$ equivariance. The process concludes with the application of a pooling layer to the $N$ dimension, culminating in a $C \times 3$ feature that adheres to $SO(3)$ equivariance.

% The fundamental challenge addressed by Vector Neurons is the inconsistent $SO(3)$ equivariance across neural network layers. Linear layers naturally exhibit equivariance: when a vector is rotated, the output of the linear layer also rotates in correspondence, thanks to the associative property of matrix multiplication. Mean pooling layers, on the other hand, inherently satisfy equivariance because when a set of vectors is rotated, the mean of the rotated vectors aligns with the rotation of the original vectors' mean, leveraging the distributive property of matrix multiplication over vector addition. This ensures that mean pooling maintains the directionality of its inputs even after rotation.

% Conversely, layers like ReLU or max pooling aren't inherently equivariant as they were primarily designed for 1-D data processing. To solve this, Vector Neurons introduce specialized operations for these layers to ensure $SO(3)$ equivariance. The traditional ReLU processes 1-D vectors and employs non-linearity based on the vector's sign. However, when dealing with 3-D inputs possessing directionality, it becomes essential to consider this directionality when applying non-linearity. Vector Neurons address this by determining the input's direction and a learned criterion. If the input's direction opposes the criterion, a projection is applied to the input vector. Likewise, for max pooling to function, it must consider the directionality when gauging input magnitudes. Vector Neurons accomplish this by training an $N$ linear layer for every $C$ channel, subsequently selecting the most optimally aligned feature from the $N$ features. As vector alignment remains invariant to rotation, rotational equivariance is thus achieved.




% \subsection{The Advantages of Equivariance}
% In this section, we organize the benefits of introducing equivariance conceretly. Equivariance can be formulated as $f_\theta(Rx)=D(R)f_\theta(x)$ where $f_\theta$ is neural network parameterized by $\theta$, $x\in \mathbb{R}^{3}$ is point, $R\in SO(3)$ is rotation matrix, and $D(R)\in \mathbb{R}^{n\times n}$ is a rotation operator for $n$ dimensional (n-D) space. 
% The equivariance property is especially helpful for the point cloud processing network because of three features.

% \textbf{Mitigation of Rotational Data Augmentation Effects.}
% Commonly, introducing rotational augmentation during training can negatively impact performance, as observed in studies like \cite{deng2021vector, puny2021frame}. Equivariance serves to neutralize this degradation, enhancing performance when datasets have been subjected to rotational perturbations. To elucidate, consider training an equivariant function $f$ for tasks like normal estimation from point clouds. Equivariance neutralizes data augmentation by ensuring that updated parameters remain consistent irrespective of whether the data points have been rotationally perturbed or not.
% Loss for tasks is $L(x,y)=\sum_id(f_{\theta}(x_i),y_i)$ where $d$ is the distance between two vectors such as squared error, and $y_i$ is the label vector for the $i$'th point. Typically, we calculate gradients $\frac{\partial L}{\partial \theta}$ to update parameters. Loss with rotated data points is $L(Rx, Ry)=\sum_id(Rf_{\theta}(x_i), Ry_i)=\sum_id(f_{\theta}(x_i), y_i)=L(x,y)$ because most distance functions are rotational invariant (i.g., $|Rx-Ry|^2_2=|x-y|^2_2$), so the gradient is same with the data points which are not perturbed by $R$. This sidesteps the typical performance decline observed with rotational data augmentation. It's important to note that this analysis remains consistent even for invariant tasks, such as shape classification.

% \textbf{Generalization Across Varied Orientations.}
% The performance of the network can be measured with certain metrics as $L(x,y)=\sum_id(f_{\theta}(x_i),y_i)$. As derived previously, this loss function remains invariant under rotation. This suggests that the performance metric remains consistent, even if the network encounters data points exclusively aligned with a canonical orientation.

% \textbf{Harmony Between Embedding and Point Space Rotations.}
% Imagine \(f\) as an encoder translating point clouds into an embedding space. The equivariance equation \(f_\theta(Rx) = D(R)f_\theta(x)\) hints that a rotation applied to the embedding \(f_\theta(x)\) mirrors a rotation applied to the input point clouds. This synchronization proves invaluable for tasks centered around pose alignment~\cite{zhu2022correspondence, fu2023neuse}, given that alignments in the embedding space can be seamlessly mirrored in the input space, i.e., the point clouds.


% \subsection{SO(3) equivariance}
% {\color{blue} Introduce equivariance here}
% description for the equivariance





% \subsection{Problem Setting}
We are interested in finding a feature representation function $\psi: \mathbb{R}^3 \rightarrow \mathbb{R}^n$ from three-dimensional feature $\vec{x} \in \mathbb{R}^3$ to high-dimensional feature $\psi(\vec{x}) \in \mathbb{R}^n$ while keeping equivariance. To define equivariance in the high-dimensional space, a mapping function $D: SO(3) \rightarrow \mathbb{R}^{n \times n}$ from a three-dimensional rotation $R \in SO(3)$ to an $n$-dimension rotation matrix $D(R) \in \mathbb{R}^{n \times n}$ should be defined. Then a feature representation function $\psi$ is $SO(3)$ equivariant if

$$\psi(R\vec{x})=D(R)\psi(\vec{x}), \quad \forall \vec{x}, \in \mathbb{R}^3 , \quad \forall R \in SO(3). $$

Although a naive feature representation, such as duplicating the input vectors $[\vec{x}, \vec{x}, \vec{x}] \in \mathbb{R}^9$, is feasible, it fails to enhance the network’s detail capture beyond using only $\vec{x}$. Therefore, it's crucial to identify the conditions that make $\psi$ effective for learning shape details and propose an algorithm to compute a $\psi$ that meets these conditions.
